SLIM: a Scalable Light-weight Root Cause Analysis for Imbalanced Data in Microservice

The newly deployed service -- one kind of change service, could lead to a new type of minority fault. Existing state-of-the-art methods for fault localization rarely consider the imbalanced fault classification in change service. This paper proposes a novel method that utilizes decision rule sets to deal with highly imbalanced data by optimizing the F1 score subject to cardinality constraints. The proposed method greedily generates the rule with maximal marginal gain and uses an efficient minorize-maximization (MM) approach to select rules iteratively, maximizing a non-monotone submodular lower bound. Compared with existing fault localization algorithms, our algorithm can adapt to the imbalanced fault scenario of change service, and provide interpretable fault causes which are easy to understand and verify. Our method can also be deployed in the online training setting, with only about 15% training overhead compared to the current SOTA methods. Empirical studies showcase that our algorithm outperforms existing fault localization algorithms in both accuracy and model interpretability.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/1-introduction-bak.tex <==
\section{Introduction}







Monolithic services have been progressively restructured into more refined modules, comprising of hundreds (or even thousands) of loosely-coupled microservices~\cite{seer,deathstar,suite,intro1}. Leading companies like Netflix, eBay and Alibaba have adopted this application model. Microservices offer several benefits that make them a powerful architecture, including simplification of application development, resource provisioning efficiency and flexibility. Despite these promising advantages, microservices introduce complex interactions among modular services, which can make on-demand resource provisioning challenging and potentially lead to performance degradation.


To enable engineers to resolve failure efficiently, fault localization is at the core of software maintenance for online service systems. With the advancement of monitoring and collecting tools, Metrics, Traces, and Logs have become the three fundamental elements of fault localization. Metrics refer to numeric data measurements taken at regular intervals of time, which help to understand the reasons behind the functioning of your application. Each trace records the process of a request being called through service instances and their operations~\cite{intro7,intro8}. Logs provide detailed information on the system's running status and user behavior. 

Though tremendous efforts have been devoted to software service maintenance and observability, in practice failures are inevitable due to the the increasing size and complexity of systems, which can result in significant economic losses and user dissatisfaction~\cite{intro1,intro2,intro3}. Analyzing the root causes of such performance issues is non-trivial and often error-prone, as hundreds of services may exhibit anomalies (e.g., network congestion and limited available cores) and propagate them to dependent services. Moreover, large microservice systems are highly active and dynamic~\cite{intro1}, with numerous service changes. 


It is important to note that the faults in a service often occur within the change of service, e.g. initial period of deploying new service or code change of services. This is due to changes in system architecture, service version (with backward or forward compatibility), and insufficient testing of the new service itself~\cite{ver1,ver2}. Google SRE book points out that about 70\% of failures are caused by changes in services~\cite{ver3}. Additionally, the lack of adequate fault data for newly deployed services hinders the learning process, making root cause analysis algorithms hard to localize such faults, leading to a chain of incidents. However, existing fault localization algorithms mainly focus on utilizing new deep-learning and machine-learning models to fully learn the information in the multi-source data (log, metric and trace), while ignoring the highly dynamic running-time status with numerous services in change. Due to the limitation of their own architecture design and model training, they are unable to quickly learn and respond to new faults caused by service changes with a small amount of fault data.



 

\textbf{Motivations.} Existing fault localization methods for imbalanced classification are roughly processed by data-level techniques by re-sampling~\cite{tracerca,dejavu}. In fact, simply over-sampling the minority class samples or down-sampling the majority class samples may cause model overfitting and on the other hand cannot generate extra insights from the data.  We show that these SOTA algorithms cannot achieve significant performance improvement through re-sampling in our experiment part~\ref{imb_exp}. Besides, many fault localization methods based on deep-learning~\cite{seer,sage,LLM} that claim to have good fault localization performance require several hours for a single training session, which fail to handle services experiencing frequent failures. In addition, these algorithms only offer simple binary classification results with a lack of interpretability, making it difficult for engineers to effectively mitigate and resolve faults even after spending a significant amount of time in root cause analysis. Therefore, how to build an interpretable fault localization model that could quickly and accurately response to newly deployed service fault patterns from a limited number of imbalanced failures is appealing but a challenging problem.


We summarize three main technical challenges to build effective fault localization models for imbalanced datasets of newly deployed services as follows.

\begin{itemize}
    \item[1)] The first challenge arises from imbalanced data of service change(e.g. newly deployed service). We also note that simply applying re-sampling does not lead performance improvement in our experiments. 
    % It is hard to be processed by data-level techniques of re-sampling.  
    \item[2)] The second challenge arises from model interpretability for operating engineers. Good interpretability can help engineers to better understand the fault cause and possibly identify related risks. Unfortunately, most of the existing works on fault localization lacks interpretability. 
    % are powerless in aiding operations personnel to quickly understand the cause of the fault.
    \item[3)] The third challenge arises from the unbearable training overhead of existing models, primarily attributed to the dynamic runtime environment in the microservice scenario.
\end{itemize}


% There are 3 primary challenges to solve when training an effective and scalable rule set model.



In this paper, we aim to design an interpretable classifier on highly imbalanced data via learning decision rule sets~\cite{CG-Dash} for fault localization. It can be expressed in disjunctive normal forms~(DNF, OR-of-ANDs), which enjoys good interpretability due to the logical clauses. An example of DNF models with two conditions is ``IF (cpu\_usage$>$80 AND file\_disk\_read$>$180) OR (file\_disk\_write$>$70 AND memory\_usage$>$170) THEN $\hat{y}=1$''. It helps engineers to understand which key metrics are affected by the fault, thus enabling the model to provide the current interpretable results. As we only focus on building rules for the minority class (further called the positive class), which makes it an ideal interpretable model for imbalanced classification. Moreover, our model can achieve incremental training within minutes for every newly deployed services, thus can be deployed to a wide range of services with low cost. 

In this paper, we propose a fault localization algorithm called \textbf{SLIM}~(\textbf{S}calable and interpretable \textbf{L}ight-weight algorithm for \textbf{I}mbalanced data in \textbf{M}icroserverice) to address the aforementioned challenges. Here we summarize the main contributions of our model as follows: 
\begin{itemize}
    
    \item To the best of our knowledge, we are the first work to address the issue of imbalanced fault data in service change(e.g.newly deployed services) from an algorithm-level within the microservices environment. Besides, our model could also handle the impact that is caused by imbalanced data between all failure samples and normal samples.

    \item Our fault localization algorithm could generate the interpretable rule set that could assist engineers in understanding the root causes of failures. %we evaluate the Label Flipping Rating这块考虑一下用什么来评估

    \item We evaluate our \textbf{SLIM}'s overhead in the three open-source dataset and the real running-time environment of cloud service system. Compared to other algorithms deployed in the system, our model's training time(12 minutes) is only around 15\% of theirs in the most complex scenarios. We confirm our model could response the newly deployed service fast enough.

    \item We conduct extensive experiments on 359 failures from three systems including three open-source datasets~\cite{dejavu}. The results show SLIM's effectiveness, efficiency and interpretability. Besides, we apply our algorithm at the real running-time of the largest cloud service system provider in China and give the case study in the part of experiment. We give the demo in the github: https://anonymous.4open.science/r/SLIM-5B7F/.


\end{itemize}






==> sections/2-relatedwork.tex <==
\section{BackGround}\label{sec:related_work}










\subsection{Basic Concepts of Microservice System}

In Figure~\ref{fig:basic}, we show the basic concepts of the microservice system. A \textbf{Microservice System} is a highly efficient architecture comprising of \textbf{Microservices} that are loosely coupled and lightweight. \textbf{Microservices} are initiated by \textbf{instances}, which is the running version of this microservice on the \textbf{Physical Node}. The status of both the \textbf{Physical Nodes} and the \textbf{Instances} are described through \textbf{metrics} generated by monitoring tools such as Prometheus~\cite{Prometheus}. The \textbf{trace} describes the execution process of a request through service instances~\cite{elasticsearch}. It has been supported by open-source solutions~\cite{jaeger,opentelemetry}. The \textbf{Logs} are produced during each service invocation, which is generated by the logging statements and records the internal status of the invocation. 



\begin{figure}
    \centering
    \includegraphics[width=1.1\linewidth]{figs/basic concepts.pdf}
    % \vspace{-15pt}
    \caption{The Overview of Microservice System.}
    \label{fig:basic}
    % \vspace{-15pt}
\end{figure}




\begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/rulesetPipelineNew.pdf}
    % \vspace{-15pt}
    \caption{The Pipeline of SLIM.}
    \label{fig:pipeline}
    % \vspace{-15pt}
\end{figure*}



\subsection{The Monitorting of Enterprise Cloud Platform}

Most enterprise operating teams use monitoring tools to observe the environment, including logs and performance metrics of hosts and applications. Microservice-based applications often utilize additional specialized monitoring, like Jaeger, which could track the RPC latency and errors between services' calls.
We describe Alibaba Cloud Observability Suite, an application-aware observability platform, which is one of our sources of experimental data(dataset D) in this paper. This platform builds an observable data layer around Prometheus~\cite{Prometheus} service, Grafana~\cite{grafana} platform, and distributed tracing service~\cite{jaeger}, enabling metric storage analysis, link storage analysis, and heterogeneous data source integration. This platform could integrate multiple data sources.
Example entity types and associated metric values are described in the table~\ref{tab:metric}. The monitoring platform also could assist us in observing the services' calling status and the detailed log information of every applications or hosts.


\begin{table}[t]
\caption{Example of Monitoring Metrics of Enterprise Cloud Platform.}
  \centering
  \begin{tabular}{c|c}
    \hline
    Entity Type & Example Metrics \\
    \hline
     & CPU utilization, memory utilization, 
    \\Container&File Disk I/O,network receive rate, 
    \\&transmit rate, network packet corrupt, \\&network packet dropped \\
    \hline
    Virtual Machine & Similar with Container metrics\\
    \hline
    Database & Login number every Seconds, 
    \\&memory utilization,CPU utilization \\
    \hline
    Physical Host & Similar with Container metrics\\
    \hline
    Switch interface & Network rate, dropped packet, latency \\
    \hline
  \end{tabular}
  \label{tab:metric}
\end{table}


 







\subsection{Prior Work of Fault Localization}

Several techniques employ the advanced data processing capabilities of machine learning and deep learning to achieve root cause analysis of multi-source data. MEPFL~\cite{MEPFL} incorporates multiple features, such as traces, configurations, and resource metrics. Three supervised machine learning models are trained using a fault injection-based training corpus to predict the root cause of microservices. Seer~\cite{seer} captures trace data at the RPC level and trains a hybrid deep learning network that combines a Convolutional Neural Network (CNN) with a Long Short-Term Memory (LSTM). The model's input and output neurons correspond to microservices, ordered in topological order from back-end microservices at the top to front-end microservices at the bottom. TraceAnomaly trys to vectorize every possible invocation paths and record their latencies. They judge the root cause by finding out the deepest service at every abnormal trace.  Dejavu~\cite{dejavu} leverages the GAT to learn the history fault and design the interpreter for their fault localization module.
% \vspace{-20pt}



% \vspace{-10pt}
\subsection{Summary and Limitations of Prior Work}

The existing deep-learning and machine-learning models are struggling to cope with such dynamic system states~\cite{icse3,icse4,icse5,icse9}. The continually increasing services make it difficult to bear the training cost of the system. Many of these models also just output the simple binary classification results that are hard to be understood by operating engineers. For example, due to the limitation of using the number of service nodes that Seer itself employs as a model input, every time a new service is deployed, the network needs to be updated again. In its paper, it mentions that when diagnosing failures for a system with 100 microservices, Seer requires nearly 90 minutes for model updating. 



\subsection{The need of handling service change}
Besides, due to the dynamic system environment, as shown in figure~\ref{fig:servicechange}, the newly deployed service faces challenges in fault localization modeling due to a lack of observable data and historical failures. This makes it difficult for the fault localization model to adequately learn the failure patterns of the service and identify faults. In the part of ~\ref{imb_exp}, we analyze the impact of the frequency of faults of a specific service in the historical training data on the accuracy of the root cause analysis algorithm. We observe that as the frequency of failures of the service increased, the accuracy of the root cause analysis algorithm improved. When there is only one instance of a fault in the training set, the performance of the root cause analysis model is poor. To deal with this problem, we try to leverage the SMOTE~\cite{chawla2002smote} and its variants~\cite{maciejewski2011local,kovacs2019smote} to create new re-samples by interpolating the minority class samples. 

Unfortunately, the data imbalanced issue exists in two situations in the system. Firstly, the proportion of normal samples is much higher than that of failure samples, and this situation can be better solved by downsampling normal samples or oversampling fault samples. Secondly, the number of failure samples in the newly deployed service is much lower than that of failure samples in other services. This situation is difficult to solve by downsampling or oversampling because the number of failure samples in the new service is too rare, and re-sampling can lead to more noise and have a negative impact on the results instead. In the part of~\ref{app:bound}, we combine the baseline models with these data re-sampling methods demonstrating that data re-sampling methods do not always work well.  


To address these problems, we propose the SLIM, an \textbf{S}calable interpretable and \textbf{L}ightweight Fault Localization for \textbf{I}mbalanced Data \textbf{M}icroservice, which trains the rule set models to solve the fault localization with the imbalanced classification problems by optimizing the F1 score subject to cardinality constraints. Our model could incrementally learn new fault types from newly deployed services at a minute-level speed on a personal computer.






\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figs/servicechange.jpg}
    % \vspace{-15pt}
    \caption{The Challenge of Service Change.}
    \label{fig:servicechange}
    \vspace{-18pt}
\end{figure}


==> sections/3-method-ori.tex <==








% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figs/rulesetPipelineNew.pdf}
%     \caption{The Pipeline of SLIM.}
%     \label{fig:pipeline}
% \end{figure*}


\section{The SLIM Algorithm}

\subsection{The Pipeline of SLIM}
SLIM is an interpretable and scalable fault localization algorithm for microservices system. It identifies the (faulty) services that cause performance degradation in a microservice system, and provides explanations for operators to understand why. Figure~\ref{fig:pipeline} shows an overview of SLIM's pipeline, primarily involving 4 modules. Firstly, it processes logs and converts them into metrics as features. Then, the features are transformed into binary encoders. With these binary features as inputs, rules can be learned. Finally, the learned rules are used to vote out faults. We will now introduce these 4 modules in detail.

\subsubsection{Log Extraction Module}
This module extracts key log information and converts it to metric data. Operational log data is in unstructured format and not suitable for direct training. So we leverage log extraction methods~\cite{scwarn} to deal with it. As Figure~\ref{fig:logparse} shows, the procedure consists of log template parsing and analysis of template variation. For the log parsing step, we first parse the normal history log messages to construct a standard template base offline using drain~\cite{drain}. These normal log templates serve as a historical reference to identify whether any new template exists in online log messages. Then we parse the online log messages too, to construct streaming time-series log templates. For the variation analysis step, streaming time-series log templates are first compared and matched with the ones in the template base. The unmatched log template, along with their quantity, types, and other features, are recorded. Finally, we aggregate these features by time interval, aligning them with the metrics' sample interval to generate a unified representation with the metrics.





\subsubsection{Feature Binarization Module}
This module generates binarized features from the metrics obtained in the feature extraction module. We employ a bucketing strategy using a sequence of thresholds to cut the numerical features into discrete, binarized features. For example, in Figure~\ref{fig:pipeline}, the network latency has a continuous distribution between 100-500ms. The data is discretized into multiple values, such as $Network\_Latency \leq 100$, $100< Network\_Latency < 200$ and $Network\_Latency \geq 200$. For categorical features, we use one-hot encoding to generate binarized features. We apply this discretization process uniformly across the data distribution. These discrete values can be combined to form rules.


\subsubsection{Efficient Rule Learning Method}
\label{sec:efficient_rule}
This module digs out the rule set by our proposed novel classifier. The algorithm first identifies rule sets for each fault type. Namely, for each fault type we train a sub-model and obtain a rule set. Then, those which hit the rules in the rule set are classified as corresponding fault samples. The detailed rule learning method will be discussed in Section~\ref{sec:detail}.


\subsubsection{Fault Localization}\label{sec:faultloc}%故障类型的定位,故障服务的定位
This module provides the final results, including the localization of fault types and the localization of fault services. We design fault ranking methods by adopting a voting mechanism that takes into account both the hit counts of each rule set and the rule's confidence. 




\subsection{Detailed Procedure of Rule Set Learning}\label{sec:detail}
In the section, we introduce our rule learning methods, including Efficient Rule Generation in Section~\ref{rulegen} and Rule Set Selection in Section~\ref{rulesel}. Before diving into the details, we first predefine some key notations.

\subsubsection{Notations and Preliminaries}
% \subsubsection{The Predefine Symbols and Information}
Given a dataset $\mathcal{X}=\{(\boldsymbol{x}_i, y_i)\}_{i=1}^n$, $\boldsymbol{x}_i\in\{0,1\}^{d}$ is 
the binary feature vector obtained from feature binarization and $y_i\in\{0,1\}$ is the true label indicating the belongingness of a given fault type. Here, $d$ is the size of the feature index set $\Gamma$. A sample $(\boldsymbol{x}_i, y_i)$ is positive if
$y_i=1 (abnormal)$ and negative if $y_i=0 (normal)$. We call the $i$-th sample is covered by feature $j$ if $x_{i,j}=1$. For example, given  $j\in d$, the $j$-th feature $Network\_delay > 200ms$, $x_{i,j}=1$ means for the $i$-th sample, $Network\_delay > 200ms$ and $x_{i,j}=0$ means $Network\_delay \leq 200ms$. Denote $h_i\in\{0, 1\}$ as the prediction of the
$i$-th sample.
For a certain fault type, we aim to predict $y$ from the dataset $\mathcal{X}$ using an interpretable rule set.

\textbf{Rule and rule set.} Our classifier is a rule set that consists of rules. We now give the definitions of these two ingredients and the related notations.
\begin{Definition}[\textbf{Rule}]\label{def:rule}
A rule $r$ is a set of feature indices, i.e. $r$ is a subset of ~$\Gamma$.
A sample $(\boldsymbol{x}_i, y_i)$ is covered by a rule $r$ if and only if $r \subseteq \{j\in \Gamma| x_{i,j}=1\}$.
\end{Definition}
\begin{Definition}[\textbf{Rule Set}]\label{def:rule set}
A rule set $s$ consists of multiple rules, and serves as a classifier,
which classifies a sample as positive if the sample is covered by at 
least one rule in $s$, and as negative if there is no rule
in $s$ that covers it. Therefore, the predicted label $h_i$ can be calculated via $\bigvee_{r\in s}(\bigwedge_{j\in r}x_{i,j})$.
\end{Definition}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/logparsing.pdf}
    \vspace{-15pt}
    \caption{Log Extraction Module: Log Parsing, Matching and Analyzing.}
    \label{fig:logparse}
    \vspace{-15pt}
\end{figure}

Let $\mathcal{X}_j$, $\mathcal{X}_r$ and $\mathcal{X}_s$ denote the set of samples covered by the $j$-th feature, the rule $r$ and the rule set $s$,
respectively. In the following we use these different subscripts to distinguish sets of samples covered by different features/rules/sets, i.e. $\mathcal{X}_j=\{i|\boldsymbol{x}_{i,j}=1\}$, $\mathcal{X}_r=\{i|(\bigwedge_{j\in r}\boldsymbol{x}_{i,j})=1\}$, $\mathcal{X}_s=\{i|\bigvee_{r\in s}(\bigwedge_{j\in r}\boldsymbol{x}_{i,j})=1\}$.
According to the relationships among the features, rules and rule sets, we get $\mathcal{X}_r=\bigcap_{j\in r}\mathcal{X}_j$
and $\mathcal{X}_s=\bigcup_{r\in s}\mathcal{X}_r$.
We define a set operator $^{+}$ as a positive sample filter, meaning that $\mathcal{X'}^+$ returns a set containing all positive samples in the arbitrary given set $\mathcal{X'}$.

\textbf{Problem Formulation.} The common evaluation metrics, accuracy and error rate, are no longer applicable in imbalanced classification as they are prone to be dominated by the majority class~\cite{Johnson2019:survey}. To address this issue, we choose F1 score instead, which combines both precision and recall and cares about the performance of the minor positive samples:
%Formally, we first derive the F1 score of a given rule set $s$.  We can represent precision and recall as $\sum_i y_i h_i / \sum_i h_i$ and $\sum_i y_i h_i / \sum_i y_i$, respectively. As a result, the F1 score can be readily computed as 
\begin{align}
    F1(s)=\frac{2\sum_i y_i h_i}{\sum_i h_i+\sum_i y_i}. 
    % \vspace{-20pt}
\end{align}
Since $\sum_i y_i h_i$ is the number of correctly classified positive samples, $\sum_i h_i$ is the number of positively predicted samples, $\sum_i h_i$, $\sum_i  y_i h_i$ and $\sum_i y_i$ 
can be rewritten as $|\mathcal{X}_s|$, $|\mathcal{X}_s^{+}|$ and $|\mathcal{X}^+|$, respectively. Formally, we formulate the F1 score as follows: 
\begin{align}
    F1(s) = \frac{2 \vert \mathcal{X}_s^+\vert}{\vert \mathcal{X}_s\vert + \vert \mathcal{X}^{+} \vert} = \frac{2 \vert \cup_{r \in s} \mathcal{X}^+_r\vert}{\vert \cup_{r \in s} \mathcal{X}_r\vert + | \mathcal{X}^+ |}. 
    \label{eqn:f1_defination}
\end{align}
To maximize F1 score, we have the following optimization problem: 
% Our objective is to train a rule set by maximizing the F1 score: 
% select certain rules from the given set of all possible rules $\Omega$ and to form a rule set that has the highest F1 score, which can be further formulated as 
\begin{align}
\begin{split}
\label{eqn:objective}
        \max\limits_{s\subseteq\Omega}& \ \frac{2 \vert \bigcup_{r \in s} \mathcal{X}^+_r\vert}{\vert \bigcup_{r \in s} \mathcal{X}_r\vert + | \mathcal{X}^+ |}, \\
    \mbox{s.t. } & \ |s| \le K, \ \Omega=\{r||r|\le l, r\subseteq\Gamma\}. 
\end{split}
\end{align}
where we set a predefined parameter $l$ to be the maximum feature length of a rule, and $K$ to be the maximum number of rules in a rule set. These constraints are to ensure the interpretablity of rules. By taking the logarithm, we can rewrite the objective in the following form:
\begin{align}
    \max \limits_{s\subseteq \Omega}\ \log (\vert \bigcup \limits_{r \in s} \mathcal{X}_r^+\vert)-\log (\vert \bigcup \limits_{r \in s} \mathcal{X}_r\vert + | \mathcal{X}^+| ).
\label{eqn:logobj}
\end{align}






% Finally, we check each sample using the learned rule set and perform a final ranking based on the fault localization method~\ref{sec:faultloc}.




\subsubsection{Rule Set Selection}\label{rulesel}
We now present the details of our efficient rule selection method. Let us rewrite the two logarithm components of \eqref{eqn:logobj} as $G(s)\triangleq\log (\vert \bigcup _{r \in s} \mathcal{X}_r^+\vert)$ and $C(s)\triangleq\log (\vert \bigcup_{r \in s} \mathcal{X}_r\vert + |\mathcal{X}^{+}|)$. 
As logarithm function is non-decreasing and concave,
both $G(s)$ and $C(s)$ are non-negative monotone submodular functions~\cite{bach2013learning}. Consequently, the objective function can be viewed as a difference between two submodular functions. 
% In this subsection, we demonstrate how SLIM selects rules.
Our proposed method, which is referred as SILM, is based on the method \textit{DistortedGreedy} \cite{harshaw2019submodular}, for maximizing
the difference between a non-negative monotone submodular function 
and a modular function. We will show that
by introducing the notation curvature, \textit{DistortedGreedy} is
applicable to our problem. We first define the curvature $\gamma$
of $C(s)$
\vspace{-.2cm}
\begin{align}
\gamma \triangleq 1-\min_{r\in\Omega}\frac{C(r|\Omega\setminus\{r\})}{C(r|\emptyset)}
\end{align}
to measure the closeness of $C(s)$ to a modular function, and $\gamma$ is unknown a priori.
The complete procedure for rule set selection is summarized in Algorithm \ref{alg:selectrules}.
Given the training dataset, the maximal number of rules and the limitation on the length of rules,
and by initializing the rule set as an empty set, we iteratively add a rule $r^{*}$ maximize a distorted marginal gain of $r$ with a parameter $\alpha$, i.e.,
\begin{align}
\label{eq:gc}
\max_{r}\quad \alpha G(r|s)-C(r|s), 
\end{align}
where $G(r|s)\triangleq G(s\cup \{r\})-G(s)$ and $C(r|s)\triangleq C(s\cup \{r\})-C(s)$ denote the marginal gains of $G$ and $C$ when adding $r$ to $s$, which is stated in line 6 of Algorithm \ref{alg:selectrules}. 

% At each iteration, we try to find a rule $r$ to maximize a distorted marginal gain of $r$ with a parameter $\alpha$. This $\alpha$ helps adjust the trade-off 
% between precision and recall. The objective becomes
% \begin{align}
% \label{eq:gc}
% \max_{|r|\le l}\quad \alpha G(r|s)-C(r|s), 
% \end{align}
% where $G(r|s)\triangleq G(s\cup \{r\})-G(s)$
% and $C(r|s)\triangleq C(s\cup \{r\})-C(s)$ denote the marginal gains of $G$ and $C$ when adding $r$ to $s$. Because $s$ is independent of $r$, \eqref{eq:gc} can be reduced to
% \begin{align}
% \max_{|r|\le l} \quad\alpha \log(|\mathcal{X}_r^{+}\cup \mathcal{X}_s^+|)-
% \log(|\mathcal{X}_r\cup \mathcal{X}_s|+|\mathcal{X}^+|).\label{eqn:obj-subproblem}
% \end{align}

\RestyleAlgo{ruled}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKw{Define}{Define}
\SetKw{Return}{Return}
\SetKw{Initialize}{Initialize}

\begin{algorithm}[ht]
\fontsize{10}{12}\selectfont
\caption{Rule Set for Imbalanced Data Set}
\label{alg:selectrules}
\textbf{Input :}Training data $\{(\boldsymbol{x}_i, y_i)\}_{i=1}^n$, cardinality $K$, curvature $\gamma$,
maximal size of a rule $l$.\\
\textbf{Output :}Rule set $s$.\\
Let $s_0 \leftarrow \emptyset$\;
\For{$i = 0,1,...,K-1$}{
    $\alpha_i \leftarrow (1-\frac{\gamma}{K})^{K-(i+1)}$\;
    $r^{*} \leftarrow \arg\max_r\; \alpha_i G(r|s)-C(r|s)$\;
    \If{$\alpha_i G(r^*|s)-C(r^*|s)>0$}{
        $s_{i+1} \leftarrow s_i \cup \{r^*\}$\;
    }
}
\Return{$ s_{K-1}$} 
\end{algorithm}
% \vspace{-15pt}


Similar to \textit{DistortedGreedy}, we adaptively update the trade-off
between $G(r|s)$ and $C(r|s)$ using $\alpha$ in line 5 of Algorithm \ref{alg:selectrules}. 
In early stages, a small value of $\alpha$ is adopted to select rules with higher \textit{precision}. The value of $\alpha$ is gradually increased to improve the \textit{recall} of the rule set.
In other words, SLIM tends to select the rules with higher \textit{precision} in the early iteration steps and focuses on the rules with higher \textit{recall} later.
The rationale behind the $\alpha$ updating strategy is that when first focusing on the rules with
high \textit{precision} and low \textit{recall}, SLIM can achieve higher precision and later improve the recall by including more rules. However, if the rules with high \textit{recall} but low \textit{precision} are given more priority in early stages, it is difficult to eliminate the effect of the false positive samples. 


To better illustrate this, we show a toy example in Figure~\ref{fig:toy_example}.
Given a dataset with 20 positive and 100 negative samples, and our goal is to select 2 rules from 3 candidate rules, namely rules A, B and C, where rule A covers 10 positive and 1 negative samples, rule B covers the rest 10 positive samples which are not covered by rule A and 1 additional negative sample, and rule C covers 18 positive samples and 5 negative samples.
We first discuss the scenario that we replace the $\alpha$ update
strategy in line 3 of Algorithm \ref{alg:selectrules} with $\alpha_i=1$.
At the first iteration for rule A, $\vert \mathcal{X}^+\vert=20$, $\vert \cup_{r \in s} \mathcal{X}_r\vert=11$, $\vert \cup_{r \in s} \mathcal{X}_r^+\vert=10$, then the marginal gain of rule A is $\log(10/(20+11))\approx \log(0.31)$.
Similarly, the marginal gains of rule B and rule C are given as $\log(10/(20+11))\approx \log(0.31)$, $\log(18/(20+18+5))\approx \log(0.42)$, respectively.
In this scenario, SLIM will select rule C in the first iteration and rule B(or A) in the second iteration. Finally, SLIM constructs 
a rule set which covers 20 positive samples and 6 negative samples.
However, with the proposed $\alpha$ update
strategy in line 3 of Algorithm \ref{alg:selectrules},
at the first iteration (corresponding to $K=2$, $i=0$, $\gamma=1$, and $\alpha=0.5$),
the marginal gains of rule A, B and C are given as $0.5 \times \log(10)-\log(31)(\approx \log(0.102))$, $0.5 \times \log(10)-\log(31)(\approx \log(0.102))$ and $0.5 \times \log(18)-\log(43)(\approx \log(0.099))$, respectively.
Then SLIM will return a better rule set that consists of rule A and rule B, which covers only $2$ negative samples.
\begin{figure}
    \centering
    \includegraphics[width=0.4\linewidth]{figs/demo.png}
    \vspace{-15pt}
    \caption{Example of the proposed rule selection strategy.}
    \label{fig:toy_example}
    \vspace{-15pt}
\end{figure}
We also give the theoretical guarantee for the proposed method at appendix~\ref{theorem:guarantee_1}











\subsubsection{Efficient Rule Generation}\label{rulegen}
Algorithm \ref{alg:selectrules} involves 
finding a rule $r$ to maximize a distorted marginal gain of $r$, i.e. solving problem (\ref{eq:gc}). 
As the number of possible rules is exponential with number of features, solving problem (\ref{eq:gc}) is NP-hard.
To address this issue, we propose an efficient rule generation method, which solves (\ref{eq:gc}) approximately.
Because $s$ is independent of $r$, (\ref{eq:gc}) can be reduced to
\begin{align}
\max_{|r|\le l} \quad\alpha \log(|\mathcal{X}_r^{+}\cup \mathcal{X}_s^+|)-
\log(|\mathcal{X}_r\cup \mathcal{X}_s|+|\mathcal{X}^+|).\label{eqn:obj-subproblem}
\end{align}
Notice that a rule $r$ is a set of feature indices, so finding an optimal rule is equivalent to finding a set of features. The expression in \eqref{eqn:obj-subproblem} can be further rewritten as:
% \begin{align}
% \begin{split}
%     W(r)\triangleq & \alpha \log(|(\cap_{j\in r}\mathcal{X}_j)^{+}\cup \mathcal{X}_s^+|)\\
% &-\log(|(\cap_{j\in r}\mathcal{X}_j)\cup \mathcal{X}_s|+|\mathcal{X}^+|).
% \end{split}\label{eqn-W}
% \end{align}
\begin{align}
% \begin{split}
    W(r)\triangleq & \alpha \log(f(r)) - \log(g(r))
    % \\
% &-\log(|(\cap_{j\in r}\mathcal{X}_j)\cup \mathcal{X}_s|+|\mathcal{X}^+|).
% \end{split}
\label{eqn-W}
\end{align}
where $f(r)\triangleq|(\cap_{j\in r}\mathcal{X}_j)^{+}\cup \mathcal{X}_s|$ and $g(r)\triangleq|(\cap_{j\in r}\mathcal{X}_j)\cup \mathcal{X}_s|+|\mathcal{X}^+|$.

Directly maximizing $W(r)$ is difficult.
Although $f(r)$
is a supermodular function, the presence of logarithm function 
makes the property of $\log(f(r))$
non-trivial(hard to optimization). In our algorithm, we leverage the MM algorithm~\cite{hunter2004tutorial} to find the trivial surrogate function for the $W(r)$ and that could iteratively increases the value and has a tight lower bound with the original $W(r)$ function.
To step further, we propose a proper lower bound of $W(r)$ by finding a lower bound of $\log(f(r))$
and an upper-bound 
of $\log(g(r))$ separately. We show the detailed procedure of finding the bound by submodular surrogate function at appendix~\ref{app:bound}. 
Leveraging the submodular surrogate function for $\log(f(r))$ and $\log(g(r))$, we could solve the F1-Score problem and improve the model's performance at imbalanced data by the trivial procedure as following.

% \textbf{Finding submodular surrogate functions of $W(r)$.} 
% We combine the bounds obtained above, and derive two tight lower bounds
% of $W(r)$ for $|r|\ge 1$ as follows,
% \begin{align}
% W(r)\ge& \alpha \log(L_{f,r^{(t)}}^{1}(r))-\frac{g(r)}{g(r^{(t)})}=V^{1}_{\alpha,r^{(t)}}(r),\\
% W(r)\ge& \alpha \log(L_{f,r^{(t)}}^{2}(r))-\frac{g(r)}{g(r^{(t)})}=V^{2}_{\alpha,r^{(t)}}(r).
% \end{align}



% \textbf{Finding Submodular Surrogate function of $\log(f(r))$.} To find a lower bound of $\log(f(r))$, we find a lower bound of $f(r)$, due to the non-decreasing property of the logarithm function. 
% Notice that it is equivalent to finding a tight upper bound of the submodular function $-f(r)$, since $f(r)$ is supersubmodular.
% Motivated by the modular upper bounds
% of submodular functions presented in \cite{nemhauser1978analysis,jegelka2011submodularity},
% two proper lower bounds of $f(r)$ are given as
% \begin{align} \label{eqn:lb4supmod1}
% L^{1}_{f, r^{(t)}}(r)\triangleq
% &f(r^{(t)})-\sum \limits_{j\in r^{(t)} \setminus r} f(j|r^{(t)} \setminus \{j\})+\sum \limits_{j \in r \setminus r^{(t)}} f(j|\emptyset)
% \nonumber\\
% \le& f(r), \ \forall\ r \subseteq \Gamma,\\
% L^{2}_{f, r^{(t)}}(r)\triangleq
% &f(r^{(t)})-\sum \limits_{j\in r^{(t)} \setminus r} f(j|\Gamma \setminus \{j\})+\sum \limits_{j \in r \setminus r^{(t)}} f(j|r^{(t)})
% \nonumber\\
% \le& f(r), \ \forall\ r \subseteq\ \Gamma,
% \end{align}
% % \begin{align}\label{eqn:lb4supmod2}
% % L^{2}_{f, r^{(t)}}(r):=
% % &f(r^{(t)})-\sum \limits_{j\in r^{(t)} \setminus r} f(j|\Gamma \setminus \{j\})+\sum \limits_{j \in r \setminus r^{(t)}} f(j|r^{(t)})\nonumber\\
% % \le& f(r), \ \forall\ r \subseteq\ \Gamma.
% % \end{align}
% where $r^{(t)}$ denotes the current estimation of $r$. These
% two inequalities hold for all possible $r^{(t)}$, and 
% the equality is achieved when $r=r^{(t)}$. 
% Since we have obtained two lower bounds of $f(r)$, 
% we have following results, 
% % the lower bounds
% % of $\log(f(r))$ can be readily obtained as $\psi(L^{1}_{f, r^{(t)}}(r))$
% % and $\psi(L^{2}_{f, r^{(t)}}(r))$.
% \begin{lemma}\label{lemma:submoudularity-lb}
% Both
% $\log(L^{1}_{f, r^{(t)}}(r))$ and $\log(L^{2}_{f, r^{(t)}}(r))$
% are submodular lower bound of $\log(f(r))$ for $|r|\ge 1$. 
% \end{lemma}




% \textbf{Finding Supmodular Surrogate function of $\log(g(r))$.}
% Next, we show how to find an upper bound of $\log(g(r))$.
% Similar to $f(r)$, $g(r)$ is also a supermodular function and we proceed to find a tight lower bound of $-g(r)$, 
% as \cite{nemhauser1978analysis,jegelka2011submodularity} also present
% a permutation-based method to find lower bounds for submodular functions.
% However, it is also mentioned in \cite{jegelka2011submodularity} that
% to certify an optimum of such a lower bound, 
% one needs to examine about $O(m)$ permutations which is critical to the algorithm, where $m$ is the size of the ground set, i.e. in our setting, $|\Gamma|$. Hence, in this paper, we employ another strategy to find an upper bound of $\log(g(r))$ by utilizing the concavity of logarithm functions.
% As $\log(x) \le \log(x_0) + \frac{1}{x_0} (x-x_0)$,
% then a tight upper bound of $\log(g(r))$ is readily given as, which holds for any $r^{(t)}$,
% \begin{align}\label{eqn:taylor}
%     \log(g(r))\le \log(g(r^{(t)}))+\frac{1}{g(r^{(t)})}(g(r)-g(r^{(t)})). 
% \end{align}
% Since such an upper bound removes the non-linearity of the
% logarithm function, it shares the same property of $g(r)$,
% which is supermodular.

% \textbf{Finding submodular surrogate functions of $W(r)$.} 
% We combine the bounds obtained above, and derive two tight lower bounds
% of $W(r)$ for $|r|\ge 1$ as follows,
% \begin{align}
% W(r)\ge& \alpha \log(L_{f,r^{(t)}}^{1}(r))-\frac{g(r)}{g(r^{(t)})}=V^{1}_{\alpha,r^{(t)}}(r),\\
% W(r)\ge& \alpha \log(L_{f,r^{(t)}}^{2}(r))-\frac{g(r)}{g(r^{(t)})}=V^{2}_{\alpha,r^{(t)}}(r).
% \end{align}

% The problem of maximizing $W(r)$ is translated 
% to maximizing $V^{1}_{\alpha}(r|r^{(t)})$ and $V^{2}_{\alpha}(r|r^{(t)})$.
% \begin{lemma}\label{lemma:submoudularity-V}
% Both $V^{1}_{\alpha}(r|r^{(t)})$ and $V^{2}_{\alpha}(r|r^{(t)})$ are
% non-monotone submodular functions. 
% \end{lemma}


% \proof
% Both $L_{f,r^{(t)}}^{1}(r)$ and $L_{f,r^{(t)}}^{2}(r)$
% are submodular, and $g(r)$ is supermodular, so both $V^{1}_{\alpha}(r|r^{(t)})$ and $V^{2}_{\alpha}(r|r^{(t)})$ are submodular functions. 
% It is obvious that $L_{f,r^{(t)}}^{1}(r)$, $L_{f,r^{(t)}}^{2}(r)$ and $g(r)$
% are all non-increasing functions, then $V^{1}_{\alpha}(r|r^{(t)})$ and $V^{2}_{\alpha}(r|r^{(t)})$ are both non-monotone functions.
% \endproof
% Maximizing a non-monotone submodular function subject to cardinality constraints has been extensively studied in the literature.
% Specifically, SLIM maximizes $V^{1}_{\alpha}(r|r^{(t)})$ and $V^{2}_{\alpha}(r|r^{(t)})$ by using a simple local search method.
% As shown in \cite{lee2010maximizing}, by identifying the cardinality constraint as a matroid constraint,
% the local search method can provide at least $1/4$-approximation to the optimum.
% \begin{lemma}
% The local search method can provide
% at least 

% $1/4$-approximation to the optimum of $V^{1}_{\alpha}(r|r^{(t)})$ and $V^{2}_{\alpha}(r|r^{(t)})$.
% \end{lemma}
% \proof See the Theorem 2.6 of \cite{lee2010maximizing}.
% \endproof

\textbf{Rule generation algorithm.} Algorithm \ref{alg:selectfeatures} summarizes our MM-based method for learning an optimal rule.
The lines 4-7 present the initialization of each MM iteration, where we insert $l$ features to an empty set greedily.
Local search is then performed to refine the solution, as stated
in lines 8-15. The replacement operation, which replaces a feature in $r$ with another feature in $\Gamma$ if the objective function can be improved, is performed in the local search procedure only. To perform the deletion operation, we extend $\Gamma$ by including the empty set, as shown in line 12 of Algorithm \ref{alg:selectfeatures}, so that a feature in $r$ can be deleted by replacing it with the empty set. To conclude, we have presented an efficient rule generating method, which
iteratively improves the objective and is guaranteed to converge
to a local optimum of the objective function. Our method illustrated in Figure~\ref{fig:toy_example} only
involves the set operation and is hence a computational efficient method. The computational complexity of our
method can be further improved by permitting early stopping, 
i.e, terminating the local search if no significant improvement is achieved by replacing features.
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/alg1.pdf}
    % \vspace{-10pt}
    \caption{Framework of Algorithm 1.}
    \label{fig:alg1}
    \vspace{-15pt}
\end{figure}

\RestyleAlgo{ruled}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKw{Define}{Define}
\SetKw{Return}{Return}
\SetKw{Initialize}{Initialize}
\SetKwFunction{GenerateRule}{GenerateRule}

\begin{algorithm}[t]
\fontsize{10}{12}\selectfont
\caption{GenerateRule}\label{alg:selectfeatures}
\textbf{Input :}$l$: Maximal size of a rule. $\alpha$: trade-off parameter.\\
\textbf{Output :} Rule $r$.\\
\Initialize{$r_0$ by \textit{GreedRatio}}\;
\For{$t=1,2,...$}{
    $r_k \leftarrow \emptyset$, $k\in\{1,2\}$\;
    \For{$i=1,2,...,l$}{
        $ j^{*} \leftarrow \mathop{\arg\max_{j \in \Gamma}}\ V_{\alpha,r^{(t-1)}}^{k}(j |r_k )$\;
        $r_k \leftarrow r_k \cup \{j^{*}\}$;
     }
    \Repeat{$\Tilde{r}=r_k$}{
        $\Tilde{r}\leftarrow r_k$\;
        \For{$i\in r_k$}
        {
            \Define{$V(j)=V_{\alpha,r^{(t-1)}}(j|r_k\setminus \{i\})$}\;
            $j^{*} \leftarrow \mathop{\arg\max_{j \in \Gamma\cup\{\emptyset\}}}\ V(j)$\;
            \lIf{$V(j^*)>0$}{$r_k \leftarrow (r_k\setminus\{i\}) \cup \{j^{*}\}$}
        }
    }
  $r^{(t)} \leftarrow \arg\max_{r\in\{r_1,r_2\}}W(r)$\;
  \lIf{$r^{(t)}=r^{(t-1)}$}{\Return{$r^{(t)}$}}
}
\end{algorithm}


% \subsubsection{Rule Set Selection}\label{rulesel}
% % In this subsection, we demonstrate how SLIM selects rules.
% Recall that as the objective (\ref{eqn:logobj}) is a difference of two submodular functions, SLIM is based on the method \textit{DistortedGreedy} \cite{harshaw2019submodular}, for maximizing
% the difference between a non-negative monotone submodular function 
% and a modular function. We will show that
% by introducing the notation curvature, \textit{DistortedGreedy} is
% applicable to our problem. We first define the curvature $\gamma$
% of $C(s)$
% \vspace{-.2cm}
% \begin{align}
% \gamma \triangleq 1-\min_{r\in\Omega}\frac{C(r|\Omega\setminus\{r\})}{C(r|\emptyset)}
% \end{align}
% to measure the closeness of $C(s)$ to a modular function, and $\gamma$ is unknown a priori.

% \begin{algorithm}[ht]
% \fontsize{10}{12}\selectfont
% \caption{Rule Set for Imbalanced Data Set}
% \label{alg:selectrules}
% \textbf{Input :}Training data $\{(\boldsymbol{x}_i, y_i)\}_{i=1}^n$, cardinality $K$, curvature $\gamma$,
% maximal size of a rule $l$.\\
% \textbf{Output :}Rule set $s$.\\
% Let $s_0 \leftarrow \emptyset$\;
% \For{$i = 0,1,...,K-1$}{
%     $\alpha_i \leftarrow (1-\frac{\gamma}{K})^{K-(i+1)}$\;
%     $r^{*} \leftarrow \GenerateRule(l,\alpha_i) $\;
%     \If{$\alpha_i G(r^*|s)-C(r^*|s)>0$}{
%         $s_{i+1} \leftarrow s_i \cup \{r^*\}$\;
%     }
% }
% \Return{$ s_{K-1}$} 
% \end{algorithm}
% % \vspace{-15pt}

% The complete procedure for rule set selection is summarized in Algorithm \ref{alg:selectrules}.
% Given the training dataset, the maximal number of rules and the limitation on the length of rules,
% and by initializing the rule set as an empty set, we iteratively add a rule $r^{*}$ to the set by invoking Algorithm \ref{alg:selectfeatures}, which is stated in line 4 of Algorithm \ref{alg:selectrules}. 
% Similar to \textit{DistortedGreedy}, we adaptively update the trade-off
% between $G(r|s)$ and $C(r|s)$ using $\alpha$ in line 3 as mentioned before Equation \eqref{eq:gc}.

% In early stages, a small value of $\alpha$ is adopted to select rules with higher \textit{precision}. The value of $\alpha$ is gradually increased to improve the \textit{recall} of the rule set.
% In other words, SLIM tends to select the rules with higher \textit{precision} in the early iteration steps and focuses on the rules with higher \textit{recall} later.
% The rationale behind the $\alpha$ updating strategy is that when first focusing on the rules with
% high \textit{precision} and low \textit{recall}, SLIM can achieve higher precision and later improve the recall by including more rules. However, if the rules with high \textit{recall} but low \textit{precision} are given more priority in early stages, it is difficult to eliminate the effect of the false positive samples. 


% To better illustrate this, we show a toy example in Figure~\ref{fig:toy_example}.
% Given a dataset with 20 positive and 100 negative samples, and our goal is to select 2 rules from 3 candidate rules, namely rules A, B and C, where rule A covers 10 positive and 1 negative samples, rule B covers the rest 10 positive samples which are not covered by rule A and 1 additional negative sample, and rule C covers 18 positive samples and 5 negative samples.
% We first discuss the scenario that we replace the $\alpha$ update
% strategy in line 3 of Algorithm \ref{alg:selectrules} with $\alpha_i=1$.
% At the first iteration for rule A, $\vert \mathcal{X}^+\vert=20$, $\vert \cup_{r \in s} \mathcal{X}_r\vert=11$, $\vert \cup_{r \in s} \mathcal{X}_r^+\vert=10$, then the marginal gain of rule A is $\log(10/(20+11))\approx \log(0.31)$.
% Similarly, the marginal gains of rule B and rule C are given as $\log(10/(20+11))\approx \log(0.31)$, $\log(18/(20+18+5))\approx \log(0.42)$, respectively.
% In this scenario, SLIM will select rule C in the first iteration and rule B(or A) in the second iteration. Finally, SLIM constructs 
% a rule set which covers 20 positive samples and 6 negative samples.
% However, with the proposed $\alpha$ update
% strategy in line 3 of Algorithm \ref{alg:selectrules},
% at the first iteration (corresponding to $K=2$, $i=0$, $\gamma=1$, and $\alpha=0.5$),
% the marginal gains of rule A, B and C are given as $0.5 \times \log(10)-\log(31)(\approx \log(0.102))$, $0.5 \times \log(10)-\log(31)(\approx \log(0.102))$ and $0.5 \times \log(18)-\log(43)(\approx \log(0.099))$, respectively.
% Then SLIM will return a better rule set that consists of rule A and rule B, which covers only $2$ negative samples.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\linewidth]{figs/demo.png}
%     \caption{Example of the proposed rule selection strategy.}
%     \label{fig:toy_example}
%     \vspace{-15pt}
% \end{figure}


% The following theorem provides a theoretical guarantee for the proposed method. 
% \begin{theorem}\label{lemma:guarantee_disgr}
% If $r^*$ in line 4 of Algorithm \ref{alg:selectrules}
% is the optimal solution of problem (\ref{eqn:obj-subproblem}), 
% Algorithm \ref{alg:selectrules} will
% return a rule set $s$ satisfying
% \begin{align}
%     G(s)-C(s)\ge (1-e^{1-\gamma})G(s^*)-C(s^*), \ |s| \le K, 
% \end{align}
% where $s^{*}$ represents the optimal solution of problem (\ref{eqn:logobj}).
% \end{theorem}
% % \proof
% % Define $q \triangleq \frac{1-\gamma}{K}$
% % and $\alpha_i \triangleq (1-q)^{K-(i+1)}$. Obviously, $\alpha_{-1}=(1-q)^K\le e^{\gamma-1}$
% % and $\alpha_{K-1}=(1-q)^0=1$. We then define
% % \begin{align}
% % &\Phi_i(T)\triangleq\alpha_{i-1}G(T)-C(T),\\
% % &\Psi_i(S_i,e)\triangleq\max(0,\alpha_i G(e|S_{i})-C(e|S_{i})).
% % \end{align}
% % Then we have
% % \begin{align}
% % &\Phi_{i+1}(S_{i+1})-\Phi_{i+1}(S_{i})\nonumber\\
% % =&\alpha_i G(S_{i+1})-C(S_{i+1})
% % -\alpha_{i-1} G(S_{i})+C(S_{i})\nonumber\\
% % =&\alpha_i G(S_{i+1})
% % -\left(1-q\right)\alpha_i G(S_{i})-C(e|S_{i})\nonumber\\
% % =&\alpha_i(G(S_{i+1})-G(S_i))
% % +q\alpha_i G(S_{i})-C(e|S_{i})\nonumber\\
% % \ge&\Psi_i(S_i,e_i)+q\alpha_i G(S_{i}). 
% % \end{align}
% % Thus, we can give a lower bound of $\Psi_i(S_i,e_i)$ as follows:
% % \begin{align}
% % &\Psi_i(S_i,e_i)\nonumber\\
% % \ge& \alpha_i G(e_i|S_{i})-C(e_i|S_{i})\nonumber\\
% % \ge&\frac{1}{K}\sum_{e\in OPT}\alpha_i G(e|S_{i})-C(e|S_{i})\nonumber\\
% % \ge&\frac{1}{K}\alpha_i(G(OPT)-G(S_{i}))
% % -\frac{1}{K}\sum_{e\in OPT}C(e|S_{i})\label{eqn:1}\\
% % \ge&\frac{1}{K}\alpha_i(G(OPT)-G(S_{i}))
% % -\frac{1}{K(1-\gamma)}C(OPT), 
% % \label{eqn:2}
% % \end{align}
% % where (\ref{eqn:1}) follows from the submodularity and monotone of $G(S)$, i.e.,
% % %其中$(*)$来自于$g(S)$的次模性及单调性，即
% % \begin{align}
% %     \sum_{e\in OPT}G(e|S_i)\ge G(OPT\cup S_i)-G(S_i)
% %     \ge G(OPT)-G(S_i).\nonumber
% % \end{align}
% % And (\ref{eqn:2}) follows from the definition of $\gamma$, i.e.,
% % %$(**)$来自于$\gamma$的定义，即
% % \begin{align}
% % &\frac{C(e|OPT\setminus e)}{C(e|\emptyset)}\ge\frac{C(e|\Omega\setminus e)}{C(e|\emptyset)}\ge1-\gamma,
% % \end{align}
% % and 
% % \begin{align}
% % \sum_{e\in OPT}C(e|S_i)&\le\sum_{e\in OPT}C(e|\emptyset)\nonumber\\
% % &\le\sum_{e\in OPT}\frac{1}{(1-\gamma)}C(e|OPT\setminus e)\nonumber\\
% % &\le\frac{1}{(1-\gamma)}C(OPT).
% % \end{align}
% % Next we prove the bound of \textit{DistortedGreedy} as follows.
% % %我们下面开始推导distorted greedy的bound
% % Note that the following equation holds: 
% % \begin{align}
% % &\Phi_0(S_0)=\alpha_{-1}G(\emptyset)-C(\emptyset)=0,\\
% % &\Phi_K(S_K)=\alpha_{k-1}G(S_K)-C(S_K)
% % =G(S_K)-C(S_K).
% % \end{align}
% % Then we have
% % \begin{align}
% % G(S_K)-C(S_K)
% % =&\Phi_K(S_K)-\Phi_0(S_0)\nonumber\\
% % =&\sum_{i=0}^{K-1}\Phi_{i+1}(S_{i+1})-\Phi_{i}(S_{i})\nonumber\\
% % \ge&\sum_{i=0}^{K-1}\Psi_i(S_i,e_i)+q\alpha_i G(S_{i})\nonumber\\
% % \ge&\sum_{i=0}^{K-1}(1-\gamma)\Psi_i(S_i,e_i)
% % +q\alpha_i G(S_{i})\label{eqn:3}\\
% % \ge&\sum_{i=0}^{K-1}(1-\gamma)(\frac{1}{K}\alpha_i(G(OPT)-G(S_{i}))\nonumber\\
% % &-\frac{1}{K(1-\gamma)}C(OPT))+q\alpha_i G(S_{i})\nonumber\\
% % \ge&\sum_{i=0}^{K-1}q\alpha_i G(OPT)-\frac{1}{K}C(OPT)\nonumber\\
% % \ge&\left(1-\left(1-q\right)^K\right)G(OPT)-C(OPT)\nonumber\\
% % \ge&(1-e^{\gamma-1})G(OPT)-C(OPT)
% % \end{align}
% % where (\ref{eqn:3}) follows from $\Psi_i(S_i,e_i)\ge0$ and $0\le(1-\gamma)\le 1$.
% % This completes the proof.
% % %We complete the whole proof here.
% % \endproof

% Theorem~\ref{lemma:guarantee_disgr} shows that although a greedy
% updating procedure is employed, Algorithm \ref{alg:selectrules}
% can still return a decent rule set once the problem (\ref{eqn:obj-subproblem})
% is solved optimally.
% Notice that, since the curvature $\gamma$ is usually unknown in advance, we run the proposed Algorithm \ref{alg:selectrules} multiple times
% with different $\gamma$ and return the rule set with best performance.

% % Finally, we check each sample using the learned rule set and perform a final ranking based on the fault localization method~\ref{sec:faultloc}.




















\subsection{Detailed procedure of Fault Localization}
In this section, we introduce the detailed procedure of fault localization. For the localization of fault type, let the $R^{*}$ denote the selected fault type result, $R$ the collection of all fault types' rule sets, $x_{i}$ the $i$-th sample in the current time period,  $r_{j}$ the $j$-th fault type and $X$ all samples. $H_{r_j}(x_i)$ is an indicator function that takes the value 1 if $x_i$ is hit by the rule set $r_j$ and 0 otherwise. If the $i$-th sample is hit by multiple rules in the $j$-th ruleset, we select the rule with the highest precision $Precision^{max}_{r_j}$ at the training set to hit the sample. So we calculate the probability of the $i$-th sample belonging to the $j$-th fault type as Equation \eqref{eq:probx} writes. Then in Equation \eqref{eq:rmax} we sum up the sample-level probability for each fault-type rule set $j$ and pick out the fault-type with the highest value as the root cause: 
\begin{align}
&P(r_{j}|x_{i})=Precision^{max}_{r_j}*H_{r_j}(x_i),\label{eq:probx}\\
&R^{*}=\underset{r_{j} \in R}{\arg\max}\sum_{x_{i} \in X}{P(r_{j}|x_{i})}. \label{eq:rmax}
\end{align}



 % to determine the final fault ranking result from the services hitting by the rule set
% $s^{*}=\underset{j \in R}{argmax}\sum_{s_{j}=0}^{c_{j}}{P(c_{j}|x_{i})}$



For the localization of service, let the $S^{*}$ denote the selected service result and $X_{k}$ all samples in the $k$-th service. $x_m \in X_{k}$ is the $m$-th sample in the $k$-th service and $H_{r_j}(x_m)$ means whether $x_m$ is hit by ruleset $r_j$. We first group the samples by service. As Equation \eqref{eq:probx2} demonstrates, similar to fault type localization, the probability for each sample is the highest precision's rule in $r_j$ when these rules in $r_j$ hits the sample and otherwise 0. Then, we individually sum up the product of all samples hit by the rules in each service multiplied by the corresponding rule precision score according to Equation \eqref{eq:rmax2}. We sort the probability results of every service and choose the service with the highest value as the root cause.

\begin{align}  
&P(r_{j}|X_{k})=\sum_{x_m \in X_{k}}{Precision^{max}_{r_j}*H_{r_j}(x_m)}\label{eq:probx2},\\
&S^{*}=\underset{X_k \in X}{\arg\max}\sum_{r_{j} \in R}{P(r_{j}|X_{k})}.\label{eq:rmax2}
\end{align}

The fault localization module could help us to confirm the failure service and fault type of the failure. We give a detailed evaluation of the effect of our model in the experiment part.








\section{The Application of interpretable ruleset}
Our interpretable ruleset could assist engineers to confirm the root cause and find out the most relevant metric for the anomaly. It makes the model could corporate with expert knowledge for troubleshooting and debugging system errors. 
On this basis, we go a step further to apply our model to generate the knowledge base for existing fault localization algorithms. We will introduce these applications in the following part.

\subsection{Overview of the Knowledge Base Generator}
Usually, an anomaly knowledge base is constructed manually to store expert experience and quickly localize history fault types. When an anomaly firstly occurs, experts analyze its key features and generate fault fingerprints for the Knowledge Base. The fingerprint will help engineers to fast solve the problem again in the future.

Therefore, expert knowledge plays an important role for many algorithms~\cite{microcbr,cloudrca}. These algorithms leverage expert knowledge to describe every fault type and construct the prior knowledge from metrics and trace data. This is called the knowledge base or case base. Although the knowledge base is necessary for real systems, it is also expensive for the company to recruit experts and build a knowledge base manually. Thus, our interpretable ruleset can help to construct the knowledge base and reduce costs.
Fig. \ref{fig:knowledgebase} shows an overview of the knowledge base generation. We try to replace the expert knowledge component in these algorithms with our rule set in order to build the knowledge base required for diagnosing faults in their models.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/KnowledgeBase-SLIM.pdf}
    \vspace{-20pt}
    \caption{The overview of Knowledge Base generation}
    \label{fig:knowledgebase}
    \vspace{-20pt}
\end{figure}

\subsection{CloudRCA}
CloudRCA~\cite{cloudrca} leverages RobustSTL to extract the abnormal metrics and identify important system metrics using the expert knowledge base. The selected metrics are learnt via a Knowledge-informed Hierarchical Bayesian Network (KHBN) to perform root cause analysis.


In our implementation, we replace the RobustSTL and expert knowledge with our interpreter to find out the most important metric sequence. We first pass labeled training data through our SLIM, where the model analyzes the fault cases to give the key ruleset. Then, we construct the feature matrix according to the ruleset including the key metric and log information. Finally, the KHBN completes the root cause analysis. We finish the experiment with the A dataset and evaluate the CloudRCA's performance.

\subsection{MicroCBR}
Similarly, we also integrate our ruleset into MicroCBR~\cite{microcbr}, which leverage the labeled anomaly case to construct the knowledge base and perform root cause analysis through case-based reasoning. Each case records a specific root cause and its solution, along with a set of anomalies detected from resource metrics, logs and other operating information. The precision of case-based reasoning is always dominated by these abnormal metrics.

We leverage our ruleset to automatically construct anomaly knowledge for its knowledge-base. First, the SLIM to learn the labeled data. 
Then, our ruleset will show the important metrics for the all fault type. MicroCBR aims to record the time-series metrics' fingerprint, which includes every key metric's spike or dip. We leverage our ruleset to assist the MicroCBR to select the key metrics and construct fingerprints.













==> sections/4-exp-bak.tex <==
\section{Experiments}\label{sec:exp}

%We perform experiments on available real-world datasets to study the proposed algorithm and compare with RF, CART and some state-of-the-art rule based models.


In this section, we perform experiments on benchmark datasets to show the performance of SLIM in comparison with the state-of-the-art fault localization algorithms. 


% In particular, we show the superior of our algorithm not only on imbalanced data but also on balanced data. 


\subsection{Experimental Setup}

\subsubsection{Datasets} We conduct experiments on three public datasets, which are denoted as dataset $\mathcal{A}$\footnote{https://github.com/NetManAIOps/DejaVu}, $\mathcal{B}$\footnote{https://github.com/NetManAIOps/DejaVu}, and $\mathcal{C}$\footnote{https://github.com/NetManAIOps/TraceRCA}, respectively.
% , and one
% real-world dataset denoted as dataset
% $\mathcal{D}$.
Dataset $\mathcal{A}$ and $\mathcal{B}$ are obtained from two different production service systems, 
which are both injected in 18 types of faults that can be summerized as: 
\one CPU exhaustion on containers, physical servers and middleware. \two packet loss, delay on service and physical node. \three database connection limit and close(just for dataset $\mathcal{A}$); \four low free memory at JVM/Tomcat (just for dataset $\mathcal{B}$); \five Disk I/O exhaustion (just for dataset $\mathcal{B}$)~\cite{dejavu}. The dataset $\mathcal{C}$ is generated by the train ticket booking microservice system~\cite{trainticket,tracerca},
where the fault classes include the network delay and CPU consuming. 
% Dataset $\mathcal{D}$ is collected from a real-world
% cloud service that deployed on a top cloud service provider.
% Deal information and experiemental results on dataset $\mathcal{D}$ can be found in the subsection \ref{csc}. 
We summerize the number of features, number of samples,
number of services, and number of faults classes
in Table~\ref{tab:fault_type}.


\begin{table}[htbp]
\caption{Details of 3 datasets.}
\begin{center}
\begin{tabular}{c c c c c}
\hline
\textbf{Dataset}&\textbf{$\#$ Features}&\textbf{$\#$ Samples}&\textbf{$\#$ Service}&\textbf{$\#$ faults classes}\\
\hline
$\mathcal{A}$&124&62249&17&18\\
$\mathcal{B}$&501&412714&29&20\\
$\mathcal{C}$&8&469988&43&2\\
% $\mathcal{D}$&64&144981&552&2\\
\hline
\end{tabular}
%\vspace{-5pt}
\label{tab:fault_type}
\end{center}
\end{table}














% \begin{table}[htbp]
% \caption{Overview accuracy comparison of root cause localization}
% \begin{center}
% \begin{tabular}{p{0.8cm} p{1.6cm} p{0.4cm} p{0.6cm} p{0.4cm} p{0.6cm} p{0.4cm} p{0.6cm}}
% \hline 
% \textbf{Dataset}&\textbf{Algorithm}&\textbf{A@1}&\textbf{A@1$\Uparrow$}&\textbf{A@2}&\textbf{A@2$\Uparrow$}&\textbf{A@3}&\textbf{A@3$\Uparrow$} \\
% \hline
%          &\textbf{SLIM} & 0.791&--\%&0.837&--\% &0.86&--\% \\
%          &DecisionTree &0.532&48.7\% &0.635&31.8\% &0.656&31.1\% \\
%          &Seer &0.482&64.1\% &0.594&40.9\% &0.643&33.7\% \\
% $\mathcal{A}$&MEPFL(RF)& 0.698&13.3\% &0.837&0\% &0.86& 0\% \\
%       &MEFPL(MLP) & 0.452 &75\% &0.574 &45.8\% &0.603 & 42.6\% \\
%         &Dejavu& 0.771&2.6\%&0.903& $-7.9$\%&0.934& $-8.6$\% \\
%         \cline{2-8}
%        & JSS'20 & 0.167&374\%&0.256&227\%&0.359& 140\%\\
%         & AutoMap & 0.336&135\%&0.435&92.4\%&0.489& 75.6\%\\
% \hline
% \hline
%          &\textbf{SLIM} & 0.673&--\%&0.75&--\%&0.827&--\%\\
%          &DecisionTree & 0.559&20.4\%&0.603&24.4\%&0.635& 30.2\%\\
%          &Seer & 0.503&33.8\%&0.564&33\%&0.603& 37.1\%\\
% $\mathcal{B}$&MEPFL(RF) & 0.698&$-3.7$\%&0.788&5.1\%&0.858& $-3.7$\%\\
%       &MEFPL(MLP) & 0.487&38.2\%&0.513&46.2\%&0.86&  $-3.8$\%\\
%         &Dejavu& 0.662&1.7\%&0.712&5.3\%&0.756& 9.4\%\\
%         \cline{2-8}
%        & JSS'20 & 0.152&343\%&0.197&281\%&0.242& 242\%\\
%         & AutoMap & 0.258&161\%&0.342&119\%&0.379& 118\%\\
% \hline
% \hline
%          &\textbf{SLIM}&0.931&--\%&0.967&--\%& 0.992 &--\% \\
%          &DecisionTree & 0.771&20.8\%&0.86&12.4\%&0.90& 10.2\%\\
%          &Seer & 0.82&13.5\%&0.843&14.7\%&0.882&12.5\%\\
% $\mathcal{C}$&MEPFL(RF)&  0.891&4.5\%&0.956&1.2\%&0.967& 2.6\%\\
%       &MEFPL(MLP) & 0.91&2.3\%&0.967&0\%&0.985&0.7\%\\
%         &Dejavu& 0.921&0.4\%&0.956&1.1\%&0.992& 0\%\\
%         \cline{2-8}
%        & JSS'20 & 0.521&78.7\%&0.837&15.5\%&0.86& 15.3\%\\
%         & AutoMap & 0.534&74.3\%&0.624&55\%&0.741&33.9\%\\
% \hline
% \hline
% % \multicolumn{8}{l}{$^{\mathrm{a}}$ A@n$\Uparrow$ refers to the percentage of \\increased accuracy over the respective methods by SLIM.}
% \end{tabular}
% \label{tab:acc}


% \end{center}
% \end{table}















\begin{table*}[htbp]
\caption{Overview accuracy comparison of root cause localization}
\begin{center}
\begin{tabular}{c c c c c c c c}
\hline 
\textbf{Dataset}&\textbf{Algorithm}&\textbf{A@1}&\textbf{A@1$\Uparrow$}&\textbf{A@2}&\textbf{A@2$\Uparrow$}&\textbf{A@3}&\textbf{A@3$\Uparrow$} \\
\hline
         &\textbf{SLIM} & 0.791&--\%&0.837&--\% &0.86&--\% \\
         &DecisionTree &0.532&48.7\% &0.635&31.8\% &0.656&31.1\% \\
         &Seer &0.482&64.1\% &0.594&40.9\% &0.643&33.7\% \\
$\mathcal{A}$&MEPFL(RF)& 0.698&13.3\% &0.837&0\% &0.86& 0\% \\
      &MEFPL(MLP) & 0.452 &75\% &0.574 &45.8\% &0.603 & 42.6\% \\
        &Dejavu& 0.771&2.6\%&0.903& $-7.9$\%&0.934& $-8.6$\% \\
        \cline{2-8}
       & JSS'20 & 0.167&374\%&0.256&227\%&0.359& 140\%\\
        & AutoMap & 0.336&135\%&0.435&92.4\%&0.489& 75.6\%\\
\hline
\hline
         &\textbf{SLIM} & 0.673&--\%&0.75&--\%&0.827&--\%\\
         &DecisionTree & 0.559&20.4\%&0.603&24.4\%&0.635& 30.2\%\\
         &Seer & 0.503&33.8\%&0.564&33\%&0.603& 37.1\%\\
$\mathcal{B}$&MEPFL(RF) & 0.698&$-3.7$\%&0.788&5.1\%&0.858& $-3.7$\%\\
      &MEFPL(MLP) & 0.487&38.2\%&0.513&46.2\%&0.86&  $-3.8$\%\\
        &Dejavu& 0.662&1.7\%&0.712&5.3\%&0.756& 9.4\%\\
        \cline{2-8}
       & JSS'20 & 0.152&343\%&0.197&281\%&0.242& 242\%\\
        & AutoMap & 0.258&161\%&0.342&119\%&0.379& 118\%\\
\hline
\hline
         &\textbf{SLIM}&0.931&--\%&0.967&--\%& 0.992 &--\% \\
         &DecisionTree & 0.771&20.8\%&0.86&12.4\%&0.90& 10.2\%\\
         &Seer & 0.82&13.5\%&0.843&14.7\%&0.882&12.5\%\\
$\mathcal{C}$&MEPFL(RF)&  0.891&4.5\%&0.956&1.2\%&0.967& 2.6\%\\
      &MEFPL(MLP) & 0.91&2.3\%&0.967&0\%&0.985&0.7\%\\
        &Dejavu& 0.921&0.4\%&0.956&1.1\%&0.992& 0\%\\
        \cline{2-8}
       & JSS'20 & 0.521&78.7\%&0.837&15.5\%&0.86& 15.3\%\\
        & AutoMap & 0.534&74.3\%&0.624&55\%&0.741&33.9\%\\
\hline
\hline
% \multicolumn{8}{l}{$^{\mathrm{a}}$ A@n$\Uparrow$ refers to the percentage of increased accuracy over the respective methods by SLIM.}
\end{tabular}
\label{tab:acc}


\end{center}
\end{table*}















% \begin{table*}[htbp]
% \caption{Overview accuracy comparison of root cause localization}
% \begin{center}
% \begin{tabular}{c c c c c c c c}
% \hline 
% \textbf{Dataset}&\textbf{Algorithm}&\textbf{A@1}&\textbf{A@1$\Uparrow$}&\textbf{A@2}&\textbf{A@2$\Uparrow$}&\textbf{A@3}&\textbf{A@3$\Uparrow$} \\
% \hline
%          &\textbf{SLIM} & 0.791&\%&0.837&\%&0.86& \%\\
%          &Decision Tree & 0.532&\%&0.635&\%&0.656& \%\\
%          &Seer & 0.482&\%&0.594&\%&0.643& \%\\
% $\mathcal{A}$&MEPFL(RF)& 0.698&\%&0.837&\%&0.86& \%\\
%       &MEFPL(MLP) & 0.452&\%&0.574&\%&0.603& \%\\
%         &Dejavu& 0.771&\%&0.903&\%&0.934& \%\\
%         \cline{2-8}
%        & JSS'20 & 0.167&\%&0.256&\%&0.359& \%\\
%         & AutoMap & 0.336&\%&0.435&\%&0.489& \%\\
% \hline
% \hline
%          &\textbf{SLIM} & 0.673&\%&0.75&\%&0.827&\%\\
%          &Decision Tree & 0.559&\%&0.603&\%&0.635& \%\\
%          &Seer & 0.503&\%&0.564&\%&0.603& \%\\
% $\mathcal{B}$&MEPFL(RF) & 0.698&\%&0.788&\%&0.858& \%\\
%       &MEFPL(MLP) & 0.487&\%&0.513&\%&0.86& \%\\
%         &Dejavu& 0.662&\%&0.712&\%&0.756& \%\\
%         \cline{2-8}
%        & JSS'20 & 0.152&\%&0.197&\%&0.242& \%\\
%         & AutoMap & 0.258&\%&0.342&\%&0.379& \%\\
% \hline
% \hline
%          &\textbf{SLIM}&0.931&\%&0.967&\%& 0.992 &\% \\
%          &Decision Tree & 0.771&\%&0.86&\%&0.90& \%\\
%          &Seer & 0.82&\%&0.843&\%&0.882& \%\\
% $\mathcal{C}$&MEPFL(RF)&  0.891&\%&0.956&\%&0.967& \%\\
%       &MEFPL(MLP) & 0.91&\%&0.967&\%&0.985& \%\\
%         &Dejavu& 0.921&\%&0.956&\%&0.992& \%\\
%         \cline{2-8}
%        & JSS'20 & 0.521&\%&0.837&\%&0.86& \%\\
%         & AutoMap & 0.534&\%&0.624&\%&0.741& \%\\
% \hline
% \hline
% \multicolumn{8}{l}{$^{\mathrm{a}}$ A@n$\Uparrow$ refers to the percentage of increased accuracy over the respective methods by SLIM.}
% \end{tabular}
% \label{tab:acc}
% \end{center}
% \end{table*}































\begin{table*}[htbp]
\small
        \centering
        \caption{An example of learned rule set of Dataset $\mathcal{A}$.}
        \begin{tabular}{c|l|c|c|c}
        \toprule
        Fault type &
        Learned rule set &Precision&Recall&\# Covered samples\\
        \midrule
        \multirow{2}{*}{\shortstack{Database Connection\\Limitation Fault}} & Login\_Per\_Sec $<$ 1.4 &100\%&45\%&18  \\
        \cline{2-5}
        & SeqRead\_Per\_Sec $>$ 1.08 $\land$ Login\_Per\_Sec\_diff $<=$ -0.10 &100\%&55\%&22 \\
        \midrule
        % Rule for &Precision&Recall&\# Covered samples\\
        % \midrule
        \multirow{2}{*}{CPU Fault}
        & proc $>$ 23.75 $\land$ count\_diff $<=$ 1042.45 &90\%&87\%&27\\
        \cline{2-5}
        &container\_cpu\_used $>$ 86.0 $\land$ count\_diff $<=$ -157.5 &100\%&11.7\%&4\\
        \bottomrule
        \end{tabular}
        \label{tbl:casestudyA}
\end{table*}








\begin{table}[htbp]
\small
        \centering
        \caption{An example of learned rule set of cloud service provider.}
        \begin{tabular}{p{3.5cm}|p{1cm}|p{0.9cm}|p{1.3cm}}
        \toprule
        Rule&Precision&Recall&\# Covered samples\\
        \midrule
        ctn\_waiting\_reason = 1.0& 63.8\%& 47.3\%&87\\
        \hline
        ctn\_status\_waiting = 1.0 $\land$ pod\_is\_scheduled = -1.0
        & 74.8\%&17.3\%&32\\
        \hline
        pod\_is\_scheduled = 0.0 $\land$ node\_ecs\_status = 0&  71.3\%&35.3\%&65\\
        \bottomrule
        \end{tabular}
        \label{tbl:casestudyali}
        \vspace{-10pt}
\end{table}









\subsubsection{Baseline Algorithms}  We compare our proposed SLIM
with several state-of-the-art fault localization algorithms, including five supervised methods, i.e. Dejavu, Seer, MEPFL-RandomForest(MEPFL-RF), Multilayer Perceptron(MEPFL-MLP) and decision tree, and two unsupervised methods, i.e. JSS'20 and AutoMap.
Dejavu is an actionable and interpretable fault localization method for recurring failures, where graph attention networks
is used to localize the fault~\cite{dejavu}. Seer~\cite{seer} captures the RPC-level graph dependency and metric by training a hybrid deep learning network that combines a CNN (Convolutional Neural Network) with an LSTM (Long Short-Term Memory). MEPFL-RandomForest(MEPFL-RF) and Multilayer Perceptron(MEPFL-MLP)~\cite{MEPFL} treat fault localization as a classification problem and solve it using traditional machine learning methods RandomForest and Multilayer Perceptron, respectively. We also compare our method with decision tree due to its interpretablity. JSS'20 represents faults as graphs and finds similar diagnosed faults by graph similarity for each incoming fault~\cite{jss20}. AutoMap leverages the multi-dimension metrics to dynamically generate service relationship graph, and then leverages the random walk algorithm to localize the fault from the graph~\cite{automap}.





\subsubsection{Parameter Tuning} We tune parameters for all methods by 5-fold cross-validation. Specifically, for our model SLIM, we choose the number of rules, i.e. parameter $K$, from $\{2, 4, 8, 12\}$, and limit the length of a rule to no more than $6$ to ensure interpretability, i.e., $l=6$.
% (we find out the $K=4$ having the best performance at three dataset).
For MEPFL-MLP and Seer, we adjust the number of neurons from [20,30,40] and the learning rate from [1e-4,5e-5,1e-5]. 
% We find out the 5e-5 and 40 neurons having best performance for these datasets.
For DecisionTree and MEPFL(RF), the number of samples at each leaf node is tuned from 1 to 100 and the number of trees is tuned in $\{1000,2000,3000\}$.
For Dejavu, we set the parameters according to the suggestion in~\cite{dejavu}.



\subsection{Performance on fault localization}

\subsubsection{Evaluation Metrics}
Top-k Accuracy, which is referred as A@k,
is used to measurement the perforemance of each methods.
Top-k Accuracy computes the probability that the root causes can be located within the top $k$ service instances among all candidates. Higher A@k indicates more accurate of the root cause localization. Here we measure the
performance of each method using $A@1$, $A@2$, and $A@3$.

\subsubsection{Performance}
We present the fault localization results in table~\ref{tab:acc}, where the result are averaged over 5 independent trials. 
% We leverage the 5-fold cross-validation and present the average results. 
% , we present the fault localization results. We leverage the 5-fold cross-validation and present the average results. 
From table~\ref{tab:acc}, we see that the proposed SLIM achieves highest Top-1 accuracy on dataset $\mathcal{A}$ and $\mathcal{A}$,
and second highest Top-1 accuracy on dataset $\mathcal{B}$. This due to we employ F1 score as objective function, which is robust to
data imbalance. In contrast, Dejavu simply resamples the data to balance the number of data in each class, thus performs slightly worse than SLIM~\cite{dejavu}. Seer, Decision Tree, MEPFL-RF, and MEPFL-MLP do not have specific designs to address imbalanced data, leading to inferior performance. 

JSS’20 and AutoMap perform poorly at three datasets. Because their approach does not make use of historical faults until the ground truths of similar historical faults are identified. Despite being carefully designed, the critical intermediate steps, such as anomaly detection methods and similarity functions, are entirely unsupervised. As a result, they may be susceptible to confusion from irrelevant abnormal changes in other metrics, which can be caused by noise or fluctuations, particularly when the number of metrics or fault units is high. On the contrary, SLIM learns to focus on the key metrics from the rule set that is generated by historical failures. 
% The traditional machine learning baselines(Decision Tree, MEPFL-RF and MEPFL-MLP) perform poorly due to the numerous useless and noisy time-series features. 


\subsubsection{Overhead}
In the Figure.~\ref{fig:overhead1}, we evaluate the training overhead for every algorithms at three datasets. As the results show, our approach has low training costs compared to all deep learning and some of machine learning models in SOTA methods. Due to the usage of LSTM and GAT in Seer and Dejavu for learning data, their training cost is much higher than other algorithms. This also means that our model can quickly learn and respond to new types of faults that may occur when this microservice system experiences service changes(e.g. the deployment of new services).

Seer and Dejavu are strongly limited by the current service topology diagram. Once there is a service change (such as deploying a new service), Seer and Dejavu cannot quickly complete accurate learning and adaptation to the new scenario. We have detailed experimental tests on this point in the later part~\ref{imb_exp}.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/overhead.pdf}
    \caption{The Overhead of All Algorithms at Three Dataset}
    \label{fig:overhead1}
    \vspace{-15pt}
\end{figure}

\subsubsection{Interpretablity}
We show the rule set learned on dataset $\mathcal{A}$ as an example in Table \ref{tbl:casestudyA}. The rule set in Table \ref{tbl:casestudyA} is to predict whether the services suffer database connection limitation or CPU fault. The learned rules imply that a service that suffers CPU fault has high CPU\_usage and process number. The service undergoes db connection limitation that has low the login user number of database per second(Login\_Per\_Sec). These rules could help the decision-makers classify a sample distinctly.



\subsection{Ability to Deal with Imbalanced Dataset}
\subsubsection{Experiment Setup}
To verify the performance advantages of our method in the data imbalance scenario, we extracted services to simulate the newly deployed services for the imbalance test. We selected the fault "network\_delay" in docker005(dataset $\mathcal{A}$), the fault "OS Network" in apache02(dataset $\mathcal{B}$) and the fault "OS Network" in Tomcat01(dataset $\mathcal{B}$). Because these faults occurs more frequently than others in the entire dataset, making it easier to characterize the trend of the fault localization performance with the frequency of occurrence. We set the test set for each service to include two faults, and the training set gradually increases from one occurrence to n-2, where n is the total number of this faults. 





\subsubsection{Numerical Results}\label{imb_exp}
In the figure~\ref{fig:imb_result}, we show three services' results of every fault localization algorithms. We find out that our model can basically learn the most critical rule information when the fault occurs for the first or second time. The other algorithms are hard to finish the fault localization from first fault happening. It means that the current system needs to experience the same fault repeatedly before the fault localization algorithm can truly accomplish fast fault localization and subsequent fault resolution processes.
Beside, we leverage the SMOTE~\cite{smote} to over-sampling the fault data from these services. We make the minority fault have the similar number to other existing faults. In the figure ~\ref{fig:imb_smote_result}, we show the result of every algorithms' performance after applying the SMOTE over-sampling method. The result is similar to the result in the figure ~\ref{fig:imb_result}. In Apache02 for Dataset B, we find out that the Seer has a little promotion. However, the SMOTE produced negative impacts for Seer at docker005 of Dataset A. We consider that the reason for this problem is due to the overfitting of the model to the data caused by oversampling of the original samples.  

% The figure also shows that when the training set continues to grow, the rules used to diagnose this type of fault remain very stable and have not changed much. This not only indicates that the rules discovered by our algorithm are very stable and critical, but also indirectly proves that our method captures the most critical fault information from the first occurrence of the fault.   



\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/imbalanced.pdf}
    \caption{The Imbalanced Dataset Experiment}
    \label{fig:imb_result}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/imbalanced_smote.pdf}
    \caption{The Imbalanced Dataset Experiment with SMOTE}
    \label{fig:imb_smote_result}
    \vspace{-15pt}
\end{figure}




%绘制训练集大小随特征




















\subsection{Performance of SLIM on Real-world system}\label{csc}
% \subsubsection{Deployment}
The cloud service system provider maintains over 5 million computers, and monitor a total of 50 million metrics in different scenarios, including cpu usage, memory usage, response
time, etc. To this end, we collect the records for each server, including system location, category and some other physical information in the most recent 30 days. We divide the dataset into two parts, each including 15 days. We want analysis the difference between the two parts, and answer the question that in which context the breakdown ratio of the servers are increased. 
We select 60+ attributes, containing the number and generation of CPU, whether there is GPU, the version of the operation system, the cluster it belongs to, the pod status, the pod is scheduled, and the server's status. To thoroughly test the performance of our model, we artificially injected 3414 faults into the cluster to simulate specific fault scenarios.





% \subsubsection{Case Study}
Table.~\ref{tbl:casestudyali} presents a case study, which shows an example of top3 patterns learned from real data. From the table, we see that SLIM discovers 3 rules in which the number of breakdown physical nodes significantly increased. As checked by business experts, the top 2 patterns are due to the increasing of daily maintenance schedule. The third pattern shows that the node's system has broken more times than 15 days ago.







==> sections/5-conclusion-bak.tex <==
\section{Conclusion}

In this paper, we propose an interpretable, effective and fast fault localization algorithm SLIM to directly optimize the F1 score, which is particularly applicable for highly imbalanced classification. Our experimental results demonstrate the superior performance and interpretability of SLIM in comparison with existing fault localization methods. In addition, the good adaptbility of SLIM makes it an ideal tool to handle large-scale microservice systems in many real-world scenarios involving frequent service change. 


% In this paper, we propose RISO for highly imbalanced data by directly optimizing the F1 score. We have shown that it achieves superior classification performance and interpretability to existing interpretable methods. With the proposed efficient implementation, our algorithm scales well on big datasets. 

%We formulate the objective as a ratio of two submodular functions which is further derived as the difference of two non-negative monotone submodular functions after a nonlinear transformation and design a novel method based on MM approach to generate rules by iteratively maximizing a non-monotone submodular lower bound.
% Through empirical studies, we have demonstrated the superior of our algorithm to random Forest and existing interpretable methods in terms of both performance and interpretability and further validated the effectiveness and scalability of our algorithm.


==> sections/Limitation.tex <==
\paragraph{Limitation And Future Work}


==> sections/discussion.tex <==

\paragraph{Discussion}
As $\vert \cup_{r \in s} \mathcal{X}_r^+\vert$
and $\vert \cup_{r \in s} \mathcal{X}_r\vert$ denote the number of positive samples and all samples
covered by the rule set $s$, respectively,
both of them are monotone, non-negative and submodular.
% Let $\phi(s)=\vert \bigcup \limits_{r \in s} \mathcal{R}^+\vert$ denote the numerator of Eq.(\ref{eqn:f1_ruleset}). $\phi(s)$ is a monotone submodular function due to the properties of the union set. Similarly the denominator is also a monotone submodular set function. 
Hence, our optimization problem can be considered as maximizing a ratio of two submodular functions subject to cardinality constraints. 
Maximizing the ratio of two non-negative monotone submodular
functions $f$ and $g$ has been investigated in the literature~\cite{pmlr-v48-baib16,perrault2021approximation}
and several methods have been proposed. Among them, \textit{GreedRatio}
is a widely used one, which greedily adds the item
with the highest ratio of marginal gains of $f$ and $g$ to the solution set.
However, \textit{GreedRatio} cannot be applied to our model as explained below. Specifically, consider adding a rule
$r'$ to the current rule set $s$, the marginal gains
of the numerator and denominator of (\ref{eqn:objective})
are given respectively as 
\begin{align}
    \vert \mathcal{X}_s^{+}\cup\mathcal{X}^+_{r'}\vert-\vert \mathcal{X}_s^{+}\vert=&\vert \mathcal{X}^{+}_{r'}\setminus\mathcal{X}_s^{+}\vert\stackrel{(a)}{=}\vert \mathcal{X}^{+}_{r'}\setminus\mathcal{X}_s\vert,\\
\vert \mathcal{X}_s\cup\mathcal{X}_{r'}\vert-\vert \mathcal{X}_s\vert=&\vert \mathcal{X}_{r'}\setminus\mathcal{X}_s\vert,
\end{align}
where equation $(a)$ comes from the fact that $\mathcal{X}_{r'}^{+}$ is a subset
of $\mathcal{X}^{+}$.
\textit{GreedRatio} selects $r'$ with the highest ratio below, 
\begin{align}
\frac{\vert \mathcal{X}_s^{+}\cup\mathcal{X}_{r'}^+\vert-\vert \mathcal{X}_s^{+}\vert}{\vert \mathcal{X}_s\cup\mathcal{X}_{r'}\vert-\vert \mathcal{X}_s\vert}
=&\frac{\vert \mathcal{X}_{r'}^{+}\setminus\mathcal{X}_s\vert}{\vert \mathcal{X}_{r'}\setminus\mathcal{X}_s\vert}
=\frac{\vert \mathcal{X}_{r'}^{+}\setminus\mathcal{X}_s\vert}{\vert \mathcal{X}_{r'}^{+}\setminus\mathcal{X}_s\vert+\vert \mathcal{X}_{r'}^{-}\setminus\mathcal{X}_s\vert}\nonumber\\
=&\frac{1}{1+\frac{\vert \mathcal{X}_{r'}^{-}\setminus\mathcal{X}_s\vert}{\vert \mathcal{X}_{r'}^{+}\setminus\mathcal{X}_s\vert}}
,
\end{align}
where 
$\vert\mathcal{X}_{r'}^{-}\setminus\mathcal{X}_s\vert=\vert\mathcal{X}_{r'}\setminus\mathcal{X}_s\vert-\vert \mathcal{X}_{r'}^{+}\setminus\mathcal{X}_s\vert$
denotes the number of negative samples newly covered by rule $r'$.
Obviously, \textit{GreedRatio} favors rules with the lowest $\vert \mathcal{X}_{r'}^{-}\setminus\mathcal{X}_s\vert/\vert \mathcal{X}_{r'}^{+}\setminus\mathcal{X}_s\vert$, which makes it prefer
the rule that covers $1$ positive samples and $0$ negative samples
over the rule that covers $1000$ positive samples and $3$ negative samples.
In other words, \textit{GreedRatio} gives higher priority to
the rule with higher precision while ignores its recall, leading to unsatisfying model generalization. 
Hence, we conclude that \textit{GreedRatio} is inappropriate to be used directly in our model.





==> sections/exp-bak.tex <==
\section{Experiments}\label{sec:exp}

%We perform experiments on available real-world datasets to study the proposed algorithm and compare with RF, CART and some state-of-the-art rule based models.


In this section, we perform experiments on benchmark datasets to study the performance of FILM in comparison with the state-of-the-art fault localization algorithms. 

% In particular, we show the superior of our algorithm not only on imbalanced data but also on balanced data. 

\subsection{Experimental Setup}









\begin{table}[htbp]
\caption{Details of 4 datasets.}
\begin{center}
\begin{tabular}{c c c c c}
\hline
\textbf{Dataset}&\textbf{Features}&\textbf{Samples}&\textbf{Service Number}&\textbf{Failure Classes}\\
\hline
$\mathcal{A}$&124&62249&17&18\\
$\mathcal{B}$&501&412714&29&20\\
$\mathcal{C}$&8&469988&43&2\\
$\mathcal{D}$&72&144981&200+&2\\
\hline
\end{tabular}
%\vspace{-5pt}
\label{tab:fault_type}
\end{center}
\end{table}





\begin{table*}[htbp]
\caption{Overview accuracy comparison of root cause localization}
\begin{center}
\begin{tabular}{c c c c c c c c c}
\hline 
\textbf{Dataset}&\textbf{Algorithm}&\textbf{Category}&\textbf{A@1}&\textbf{A@1$\Uparrow$}&\textbf{A@2}&\textbf{A@2$\Uparrow$}&\textbf{A@3}&\textbf{A@3$\Uparrow$} \\
\hline
         &\textbf{FILM} &Supervised& 0.791&\%&0.837&\%&0.86& \%\\
         &Decision Tree &Supervised& 0.532&\%&0.635&\%&0.656& \%\\
         &Seer &Supervised& 0.482&\%&0.594&\%&0.643& \%\\
$\mathcal{A}$&MEPFL(RF)& Supervised & 0.698&\%&0.837&\%&0.86& \%\\
      &MEFPL(MLP) &Supervised& 0.452&\%&0.574&\%&0.603& \%\\
        &Dejavu&Supervised& 0.771&\%&0.903&\%&0.934& \%\\
       & JSS'20 & Unsupervised& 0.167&\%&0.256&\%&0.359& \%\\
        & AutoMap & Unsupervised& 0.336&\%&0.435&\%&0.489& \%\\
\hline
         &\textbf{FILM} &Supervised& 0.673&\%&0.75&\%&0.827&\%\\
         &Decision Tree &Supervised& 0.559&\%&0.603&\%&0.635& \%\\
         &Seer &Supervised& 0.503&\%&0.564&\%&0.603& \%\\
$\mathcal{B}$&MEPFL(RF)& Supervised & 0.698&\%&0.788&\%&0.858& \%\\
      &MEFPL(MLP) &Supervised& 0.487&\%&0.513&\%&0.86& \%\\
        &Dejavu&Supervised& 0.662&\%&0.712&\%&0.756& \%\\
       & JSS'20 & Unsupervised& 0.152&\%&0.197&\%&0.242& \%\\
        & AutoMap & Unsupervised& 0.258&\%&0.342&\%&0.379& \%\\
\hline
         &\textbf{FILM}&Supervised&0.931&\%&0.967&\%& 0.992 &\% \\
         &Decision Tree &Supervised& 0.771&\%&0.86&\%&0.90& \%\\
         &Seer &Supervised& 0.82&\%&0.843&\%&0.882& \%\\
$\mathcal{C}$&MEPFL(RF)& Supervised & 0.891&\%&0.956&\%&0.967& \%\\
      &MEFPL(MLP) &Supervised& 0.91&\%&0.967&\%&0.985& \%\\
        &Dejavu&Supervised& 0.921&\%&0.956&\%&0.992& \%\\
       & JSS'20 & Unsupervised& 0.521&\%&0.837&\%&0.86& \%\\
        & AutoMap & Unsupervised& 0.534&\%&0.624&\%&0.741& \%\\
\hline
\multicolumn{9}{l}{$^{\mathrm{a}}$ \textbf{A@n} means top-k accuracy, A@n$\Uparrow$ refers to the percentage of FILM' increased accuracy}
\end{tabular}
\label{tab:acc}


\end{center}
\end{table*}








\begin{table*}[htbp]
        \centering
        \caption{An example of learned rule set of Dataset $\mathcal{A}$.}
        \begin{tabular}{l|c|c|c}
        \toprule
        Rule for Database Connection Limitation Fault&Precision&Recall&Cover samples\\
        \midrule
        Login\_Per\_Sec $<$ 1.4 &100\%&45\%&18  \\
        SeqRead\_Per\_Sec $>$ 1.08 AND Login\_Per\_Sec\_diff $<=$ -0.10 &100\%&55\%&22 \\
        \midrule
        Rule for CPU Fault&Precision&Recall&Cover samples\\
        \midrule
        proc $>$ 23.746190350000006 AND count\_diff $<=$ 1042.450000000002 &90\%&87\%&27\\
        container\_cpu\_used $>$ 86.0 AND count\_diff $<=$ -157.49999999999994 &100\%&11.7\%&4\\
        \bottomrule
        \end{tabular}
        \label{tbl:casestudyA}
\end{table*}








\begin{table}[htbp]
        \centering
        \caption{An example of learned rule set of cloud service provider.}
        \begin{tabular}{l|c|c|c}
        \toprule
        Rule&Precision&Recall&Covered samples\\
        \midrule
        ctn\_waiting\_reason=1.0& 63.8\%& 47.3\%&87\\
        ctn\_status\_waiting=1.0 AND pod\_is\_scheduled=-1.0& 74.8\%&17.3\%&32\\
        pod\_is\_scheduled=0.0 AND node\_ecs\_status=0&  71.3\%&35.3\%&65\\
        \bottomrule
        \end{tabular}
        \label{tbl:casestudyali}
\end{table}









\subsubsection{Baseline Algorithms}  We compare several state-of-the-art fault localization algorithms: 
\one Dejavu designs a deep learning-based model based on graph attention networks to localize the fault~\cite{dejavu}. \two Seer, which is based CNN and LSTM~\cite{seer}. It captures the RPC-level graph dependency and metric to train a hybrid deep learning network that combines a CNN (Convolutional Neural Network) with an LSTM (Long Short-Term Memory). \three JSS'20 represents failures as graphs and finds similar diagnosed failures by graph similarity for each incoming failure~\cite{jss20}. \four Traditional machine learning models, including Decision Tree, MEPFL-RandomForest(MEPFL-RF) and Multilayer Perceptron(MEPFL-MLP)~\cite{MEPFL-MLP}. \five AutoMap leverages the multi-dimension metrics to dynamically generate service relationship graph. Then, leveraging the random walk algorithm to localize the fault from the graph~\cite{automap}.





\subsubsection{Parameter Tuning}We tune parameters for all methods by 5-fold cross-validation. Specifically, for our model: \textbf{FILM}, we choose the parameter $K$ (number of rules) from $\{2, 4, 8, 12\}$, and limit the length of a rule to $6$ for better interpretability, i.e., $l=6$. finally, we find out the $K=4$ having the best performance at three dataset and could give enough interpretability.
For Dejavu, we obey their default setting about hyperparameters due to Dejavu already testing the performance at these datasets. 
For MEPFL(MLP) and Seer, we adjust the number of neurons from [20,30,40] and the learning rate from [1e-4,5e-5,1e-5]. We find out the 5e-5 and 40 neurons having best performance for these datasets.
For DecisionTree and MEPFL(RF), the number of samples at each leaf node is tuned from 1 to 100 and the number of trees is tuned in $\{1000,2000,3000\}$.





\subsubsection{Imbalanced Experiment Setup}
To verify the performance advantages of our method in the data imbalance scenario, we extracted services to simulate the newly deployed services for the imbalance test. We selected the fault "network\_delay" in docker005(dataset $\mathcal{A}$), the fault "OS Network" in apache02(dataset $\mathcal{B}$) and the fault "OS Network" in Tomcat01(dataset $\mathcal{C}$). Because these failures occurs more frequently than others in the entire dataset, making it easier to characterize the trend of the fault localization performance with the frequency of occurrence. We set the test set for each service to include two failures, and the training set gradually increases from one occurrence to n-2, where n is the total number of this failures. Besides, due to the limitation of the number of faults, we no longer use the method of aggregating data from each fault time period to output top-k rankings (A@1,A@2,A@3). Instead, we individually calculate all fault samples that appear in each fault time period and use precision to determine which algorithm can diagnose the most fault samples. For example, one of the fault "network\_delay" in docker005 during 5 minutes, generates 5 fault samples. The fault occurs ten times total and could generate 50 fault samples.



\subsection{Experiment Result}

\subsubsection{Performance}
In table~\ref{tab:acc}, we present the fault localization results. We leverage the 5-fold cross-validation and present the average results. 

JSS’20 and AutoMap perform poorly at three datasets. Because their approach does not make use of historical failures until the ground truths of similar historical failures are identified. Despite being carefully designed, the critical intermediate steps, such as anomaly detection methods and similarity functions, are entirely unsupervised. As a result, they may be susceptible to confusion from irrelevant abnormal changes in other metrics, which can be caused by noise or fluctuations, particularly when the number of metrics or failure units is high. On the contrary, FILM learns to focus on the key metrics from the rule set that is generated by historical failures.  

The traditional machine learning baselines perform poorly due to the 


\subsubsection{Overhead}
In the Figure.~\ref{fig:overhead1}, we evaluate the training overhead for every algorithms at three datasets. As the results show, our approach has low training costs compared to all deep learning and some of machine learning models in SOTA methods. Due to the usage of LSTM and GAT in Seer and Dejavu for learning data, their training cost is much higher than other algorithms. This also means that our model can quickly learn and respond to new types of faults that may occur when this microservice system experiences service changes(e.g. the deployment of new services).

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/overhead.pdf}
    \caption{The Overhead of All Algorithms at Three Dataset}
    \label{fig:overhead1}
\end{figure}


\subsubsection{Imbalanced Experiment Result}
In the figure~\ref{imb_result}, we show three services' results of every fault localization algorithms. We find out our model could 

%绘制训练集大小随特征

\subsubsection{Interpretable Experiment Result}
We show the rule set learned on dataset $\mathcal{A}$ as an example in Table \ref{tbl:casestudyA}. The rule set in Table \ref{tbl:casestudyA} is to predict whether the services suffer database connection limitation or CPU fault. The learned rules imply that a service that suffers CPU fault has high CPU\_usage and process number. The service undergoes db connection limitation that has low the login user number of database per second(Login\_Per\_Sec). These rules could help the decision-makers classify a sample distinctly.


















\subsection{Case Study of the cloud service system provider}
\subsubsection{Deployment}
The cloud service system provider maintains over 5 million computers, and monitor a total of 50 million metrics in different scenarios, including cpu usage, memory usage, response
time, etc. To this end, we collect the records for each server, including system location, category and some other physical information in the most recent 180 days. Especially, 60+ attributes are selected, containing the number and generation of CPU, whether there is GPU, the version of the operation system, the cluster it belongs to, the pod status, the pod is scheduled, and the server's status. To thoroughly test the performance of our model, we artificially injected 3414 faults into the cluster to simulate specific fault scenarios.





\subsubsection{Case Study}
Table.~\ref{tbl:casestudyali} presents a case study, which shows an example of top3 patterns learned from real data. From the table, we see that FILM discovers 3 rules in which the number of breakdown physical node significantly increased. As checked by bussiness experts, the top 2 patterns are due to the increasing of daily maintenance schedule. The third pattern shows that the system broken more times than 90 days ago.





Besides, our model could finish the fault localization 


==> sections/formulation.tex <==
% \section{Problem Formulation}\label{sec:problem formula}
% Without loss of generality, in this paper we focus on binary classification problems with highly imbalanced data, where the number of samples of one class is much smaller than that of the other. Also we assume all features are binary features. 
% % Note that numerical and categorical features can be easily binarized using discretization and one-hot encoding respectively.
% Note that the categorical features can be easily binarized using one-hot encoding. For numeric features, here we use a sequence of thresholds to compare with the numerical features to generate binarized features, which is also known as bucketing strategy.

% Formally, given a dataset $\mathcal{X}=\{(\boldsymbol{x}_i, y_i)\}_{i=1}^n$ with a feature index set $\Gamma$ of size $d$, where 
% $\boldsymbol{x}_i\in\{0,1\}^{d}$ and $y_i\in\{0,1\}$ denote 
% the binary feature vector and the label of the $i$-th sample, respectively.
% Assuming that a sample $(\boldsymbol{x}_i, y_i)$ is positive if
% $y_i=1$ and negative if $y_i=0$.
% We aim to learn an interpretable rule set from the dataset $\mathcal{X}$.

% \begin{Definition}[\textbf{Rule}]\label{def:rule}
% A rule $r$ is a set of feature indices, i.e. $r$ is a subset of $\Gamma$.
% A sample $(\boldsymbol{x}_i, y_i)$ is considered to be covered by a rule $r$ if and only if $r \subseteq \{j\in \Gamma| x_{i,j}=1\}$.
% \end{Definition}
% \begin{Definition}[\textbf{Rule Set}]\label{def:ruleset}
% A rule set $s$ consists of multiple rules, and serves as a classifier,
% which classifies a sample as positive if the sample is covered by at 
% least one rule in $s$, and as negative if there is no rule
% in $s$ that covers it, i.e., predict the label of 
% $\boldsymbol{x}_i$ as $\bigvee_{r\in s}(\bigwedge_{j\in r}x_{i,j})$.
% \end{Definition}
% % To better illustrate our method, we define the notation \textit{cover set} for
% % features, rules and rulesets, respectively, as follows.

% % The set of samples covered by $j$th feature is defined as $\mathcal{E}=\{i|x_{i,j}=1\}$.
% % The set of samples covered by a rule $r$ is $\mathcal{R}=\{i|(\bigwedge_{j\in r}x_{i,j})=1\}$.
% % The set of samples covered by a ruleset $s$ is $\mathcal{S}=\{i|\bigvee_{r\in s}(\bigwedge_{j\in r}x_{i,j})=1\}$.
% % , and 
% % a rule, $r$, is a set of feature indices, i.e. $r$ is a subset of $\Gamma$.
% % A sample $(\boldsymbol{x}_i, y_i)$ is considered to be covered by a rule $r$ if and only if $r \subseteq \{j\in \Gamma| \boldsymbol{x}_{i,j}=1\}$.
% % We also consider a sample $(\boldsymbol{x}_i, y_i)$ to be covered by
% % the $j$-th feature if $x_{i,j}=1$.
% % A rule set $s$ serves as a classifier here,
% % which classifies a sample as positive if the sample is covered by at least one rule 
% % in $s$, and as negative if there is no rule
% % in $s$ that covers it. 
% % A sample is also called ``covered by a rule set''
% % if it is classified as positive. 
% Let $\mathcal{X}_j$, $\mathcal{X}_r$ and $\mathcal{X}_s$ denote the set of samples covered by the $j$-th feature, the rule $r$ and the rule set $s$,
% respectively. Note that in the following we may use different subscripts to distinguish sets of samples covered by different features/rules/sets. Thus, we can write $\mathcal{X}_j=\{i|\boldsymbol{x}_{i,j}=1\}$, $\mathcal{X}_r=\{i|(\bigwedge_{j\in r}\boldsymbol{x}_{i,j})=1\}$, $\mathcal{X}_s=\{i|\bigvee_{r\in s}(\bigwedge_{j\in r}\boldsymbol{x}_{i,j})=1\}$.
% According to the relationships among the features, rules and rule sets, we get $\mathcal{X}_r=\cap_{j\in r}\mathcal{X}_j$
% and $\mathcal{X}_s=\cup_{r\in s}\mathcal{X}_r$.
% Let $\mathcal{X}^+$ be the set of all positive samples in the dataset $\mathcal{X}$, we define the operation $\mathcal{A}^{+}$ as $\mathcal{A}^{+}=\mathcal{A} \cap \mathcal{X}^+$ for any set $\mathcal{A}$, which returns the set of all positive samples in $\mathcal{A}$.

% It is well-known that accuracy and error rate, the most frequently used metrics in classification evaluation, are not applicable in imbalanced classification as they are dominated by the majority class~\cite{Johnson2019:survey}. In this paper, we  
% %The drawback of only considering the model \textit{precision} when dealing with imbalanced datasets has been extensively studied.
% %Thus in this work, we 
% learn a rule set by directly maximizing the F1 score, which combines both precision and recall in classification evaluation. 
% % which has been widely used as a metric of model performance for imbalanced datasets.
% Formally, we first derive the F1 score of a given rule set $s$. 
% Let $y_i\in\{0,1\}$ and $h_i\in\{0, 1\}$ denote the true label and the prediction of the
% $i$-th sample, respectively. We can represent precision and recall as $\sum_i y_i h_i / \sum_i h_i$ and $\sum_i y_i h_i / \sum_i y_i$, respectively. As a result, the F1 score can be readily computed as 
% \begin{align}
%     F1(s)=\frac{2\sum_i y_i h_i}{\sum_i h_i+\sum_i y_i}. 
% \end{align}
% Note that the term $\sum_i y_i h_i$ denotes the number of positive
% samples that are correctly classified by our model, and
% the term $\sum_i h_i$ denotes the number of all samples
% that are predicted as positive by our model. Thus
% $\sum_i h_i$, $\sum_i  y_i h_i$ and $\sum_i y_i$ 
% can be rewritten as $|\mathcal{X}_s|$, $|\mathcal{X}_s^{+}|$ and $|\mathcal{X}^+|$, respectively. Formally, we formulate the F1 score as follows: 
% \begin{align}
%     F1(s) = \frac{2 \vert \mathcal{X}_s^+\vert}{\vert \mathcal{X}_s\vert + \vert \mathcal{X}^{+} \vert} = \frac{2 \vert \cup_{r \in s} \mathcal{X}^+_r\vert}{\vert \cup_{r \in s} \mathcal{X}_r\vert + | \mathcal{X}^+ |}. 
%     \label{eqn:f1_defination}
% \end{align}
% In this paper, our goal is to learn an interpretable and simple rule set with maximal F1 score. Formally, we have the following optimization problem: 
% % Our objective is to train a rule set by maximizing the F1 score: 
% % select certain rules from the given set of all possible rules $\Omega$ and to form a rule set that has the highest F1 score, which can be further formulated as 
% \begin{align}
%     \max\limits_{s\subseteq\Omega}& \ \frac{2 \vert \cup_{r \in s} \mathcal{X}^+_r\vert}{\vert \cup_{r \in s} \mathcal{X}_r\vert + | \mathcal{X}^+ |}, \label{eqn:objective}\\
%     \mbox{s.t. } & \ |s| \le K,\nonumber\\
%     & \ \Omega=\{r||r|\le l, r\subseteq\Gamma\}. \nonumber
% \end{align}
% To ensure the interpretablity of rules, we consider both the number of rules and the length of rules. Specifically, we require all rule lengths are no more than $l$, i.e., $|r|\le l,\ \forall r\subseteq\Gamma$, where $l$ is a predefined parameter, $\Gamma$ is the feature index set with size $d$. Also we add a cardinality constraint $|s| \le K$ to ensure that there are no more than $K$ rules in the rule set.


